On the Effect of Defections in Federated Learning and How to Prevent Them

Federated learning is a machine learning protocol that enables a large population of agents to collaborate over multiple rounds to produce a single consensus model. There are several federated learning applications where agents may choose to defect permanently$-$essentially withdrawing from the collaboration$-$if they are content with their instantaneous model in that round. This work demonstrates the detrimental impact of such defections on the final model's robustness and ability to generalize. We also show that current federated optimization algorithms fail to disincentivize these harmful defections. We introduce a novel optimization algorithm with theoretical guarantees to prevent defections while ensuring asymptotic convergence to an effective solution for all participating agents. We also provide numerical experiments to corroborate our findings and demonstrate the effectiveness of our algorithm.

==> flowchart.tex <==

\tikzstyle{startstop} = [rectangle, rounded corners, 
minimum width=3cm, 
minimum height=1cm,
text centered, 
text width=6.2cm, 
draw=black, 
fill=red!30]

\tikzstyle{io} = [trapezium, 
trapezium stretches=true, % A later addition
trapezium left angle=70, 
trapezium right angle=110, 
minimum width=3cm, 
minimum height=1cm, text centered, 
draw=black, fill=blue!30]

\tikzstyle{process} = [rectangle, rounded corners, 
minimum width=3cm, 
minimum height=1cm,
text centered, 
text width=6cm, 
draw=black, 
fill=blue!30]

\tikzstyle{process2} = [rectangle, rounded corners, 
minimum width=3cm, 
minimum height=0.8cm,
text centered, 
text width=3cm, 
draw=black, 
fill=blue!30]

\tikzstyle{decision} = [diamond, 
minimum width=2cm, 
minimum height=1cm, 
text centered, 
aspect=2,
draw=black, 
fill=green!30]
\tikzstyle{arrow} = [thick,->,>=stealth]


\begin{tikzpicture}[node distance=2cm]

\node (start) [startstop] {the server sends the synchronized model $w_{r-1}$ to all remaining agents $\mmm_{r-1}$};
\node (pro1) [process, below of=start, yshift=0.3cm] {Agents $m\in \mmm_{r-1}$ evaluate their loss $F_m(w_{r-1})$};
\node (dec1) [decision, below of=pro1, yshift=-0.1cm] {If $F_m(w_{r-1})\leq \epsilon$?};
\node (pro2a) [process, below of=dec1, yshift=-0.3cm] {Let $\cM_r\subseteq \cM_{r-1}$ denote the set of agents who want to stay. For each $m\in \cM_r$, agent $m$ sends $\ooo_m(w_{r-1})$ back to the server};
\node (pro2b) [process2, right of=dec1, xshift=1.7cm, rotate =270] {Agent $m$ defects};
% \node (out1) [io, below of=pro2a] {Output};
\node (stop) [startstop, below of=pro2a, yshift=-0.1cm] {The server aggregates the model by $w_r = w_{r-1} - \eta_r \cdot h_r\rb{\{\ooo_m(w_{r-1})\}_{m\in \cM_r}}$
    };

\draw [arrow] (start) -- (pro1);
\draw [arrow] (pro1) -- (dec1);
\draw [arrow] (dec1) -- node[anchor=east] {no} (pro2a);
\draw [arrow] (dec1) -- node[anchor=south] {yes} (pro2b);
\draw [arrow] (pro2a) -- (stop);


\end{tikzpicture}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> src/alg-backup.tex <==
% \todohs{maybe move the current remark to motivate the idea of providing a bad model to agents with low loss}
% \begin{remark}
%     Notice that the defection depends on the loss function and the synchronized model provided by the server.
%     Suppose that the loss $f(w;(x,y)) = -(2y-1)w^\top x$ is a linear function. Then the local update on each machine is an accumulation of local data which does not depend on the given model! 
%     Thus the server can cheat by sending each agent a fake model $w^m_{rK} =\bZero$ for $rK<T$ and no agent will defect if $\bZero$ is not a good model.
%     Once the server collects enough data, it outputs the true synchronized model in the final round.
% \end{remark}
% \todohs{Add a brief description on the potential method as we discussed}

In this section, we present our method, i.e., \textsc{ADA-GD}, in Algorithm \ref{alg:reweight}. At our method's core is an adaptive aggregation approach for the gradients received from agents, which disincentivizes participating agents' defection during the training. Before we state our algorithm, let's recall the definition of the orthogonal complement of a subspace. 
\begin{definition}[Orthogonal complement]
    Let $V$ be a vector space with an inner-product $\inner{\cdot}{\cdot}$. For any subspace $U$ of $V$, we define the orthogonal complement as $U^\perp := \{v\in V: \inner{v}{u} = 0,\ \forall u\in U\}$. We also define the projection operator onto a subspace $U$ by $\Pi_{U}:V\to U$. 
\end{definition}

\begin{algorithm}[t]\caption{Adaptive Defection-aware Aggregation for Gradient Descent (\textsc{ADA-GD})}\label{alg:reweight}
\textbf{Parameters:} step size $\eta$, initialization $w_{0}$\\
    % Initialize at $w_{0}$\\
    \If{$\exists m\in[M], \text{ s.t. }F_m(w_0)\leq \epsilon$}{
    STOP \Comment{Case 0\hs{to remove}}
    } 
    \For{$t=1,2,\ldots$}{
    Compute $\nabla F_m(w_{t-1})$ for all $m\in[M]$\\
    \textbf{Predict defecting agents:} $D = \{m\in[M]: F_m(w_{t-1}) - \eta\norm{\nabla F_m(w_{t-1})}\leq 2\epsilon\}$\label{alg-step:defecting}\\ 
    \textbf{Predict non-defecting agents:} $ND = [M]\setminus D$\label{alg-step:non-defecting}\\
    \If{Both $D$ and $ND$ are non-empty}{
    Compute $\nabla F_{ND}(w_{t-1}) = \sum_{m\in ND}\nabla F_m(w_{t-1})$\\
    Let $P = Span\{\nabla F_n(w_{t-1}): n\in D\}^\perp$\\
    \If{$\norm{\Pi_P\rb{\nabla F_{ND}(w_{t-1})}}\neq 0$}{
    Project $\nabla F_{ND}(w_{t-1})$ and normalize $\ngrad{ND}(w_{t-1}) = \frac{\Pi_P\rb{\nabla F_{ND}(w_{t-1})}}{\norm{\Pi_P\rb{\nabla F_{ND}(w_{t-1})}}}$\\
    $g_t = -\min\cb{\norm{\Pi_P\rb{\nabla F_{ND}(w_{t-1})}}, 1}\cdot\ngrad{ND}(w_{t-1})$\Comment{Case 1.a}\\
    }
    \Else{
    \If{$\nabla F_{ND}(w_{t-1})=0$}{
    \Return $\hat{w} = w_{t-1}$ \Comment{Case 1.b\hs{tr}}\\
    }
    \Else{
    STOP \Comment{Case 1.c\hs{tr}}\\
    }
    }
    }
    \If{$D$ is empty}{
    \If{$\nabla F(w_{t-1})\neq 0$}{
    $g_t = -\min\{\norm{\nabla F(w_{t-1})}, 1\}\cdot\frac{\nabla F(w_{t-1})}{\norm{\nabla F(w_{t-1})}}$ \Comment{Case 2.a}\\
    }
    \Else{
    \Return $\hat{w} = w_{t-1}$ \Comment{Case 2.b\hs{to remove}}
    }
    }
    %\\
    \If{$ND$ is empty }{
    \Return $\hat{w} = w_{t-1}$ \Comment{Case 3}
    }
    $w_t = w_{t-1} + \eta g_t$
    }
    
\end{algorithm}
\paragraph{Algorithm design.}
% \noindent\textbf{Algorithm design.} 
According to Algorithm \ref{alg:reweight}, the server will first predict defecting and non-defecting agents at each iteration, given the current information received from agents (see lines~\ref{alg-step:defecting}-\ref{alg-step:non-defecting}). If no agent defects, the server will normalize the aggregated gradient and use it to update the current model (see line 19 to line 23).  If all the agents defect, the server will output the current model as the final model (see line 25). Suppose there exist both defecting and non-defecting agents. In that case, the server will aggregate the gradients from non-defecting agents and project them to the orthogonal complement of the space spanned by the gradients of the defecting agents. Then, the server will update the current model using the normalized projected gradients (see line 8 to line 18). Note that Algorithm \ref{alg:reweight} fits in the class of ICFO algorithms specified by Algorithm \ref{alg:icfo}, as orthogonalization and normalization returns an output that is in the linear span of the machines' gradients. In Figure \ref{fig:our_algorithm}, we compare \textsc{ADA-GD} against \textsc{FedAvg}, demonstrating the benefit of adaptive aggregation. Next, we will provide the convergence guarantee of Algorithm \ref{alg:reweight}. We first introduce the following heterogeneity assumption implying that the functions are \textit{``dissimilar enough''}. 
% This is almost without loss of generality as for applications such as cross-device federated learning, we want to pick a representative and diverse set of devices that are not replaceable by other devices in the selection.
\begin{assumption}[Minimal Heterogeneity]\label{ass:hetero}
    Consider differentiable functions $\{F_m:\rr^d\to \rr\}$. Then for all $w\in \www\setminus \www^\star$, all non-zero vectors in $\{\nabla F_m(w): m\in[M]\}$ are linearly independent.
\end{assumption}

Remark on Assumption~\ref{ass:hetero}. Without Assumption~\ref{ass:hetero}, defection is unavoidable. 
Consider a simple two-dimensional example where $F_1(w) = \norm{w}^2$ and $F_2 = \epsilon\norm{w}^2$. Whenever we reach some $w_t$ with $\norm{w_t}^2\in (0.1, 1]$, agent $2$ will defect.


\begin{equation*}
    F_2(w)
\end{equation*}

$F_2(w) = \epsilon\norm{w}^2$ for $w\in \R^2$. In the optimization process, if at time $t$ we have $\norm{w_t} =1$, then agent 2 defects

there exists a time step that Then on the optimizing trajectory optimizing at any $w$ with $\norm{w} = 1$

\begin{lemma}\label{lem:ass_hetero}
    Suppose Assumption \ref{ass:hetero} holds. For all $A\subset [M]$ and $B = [M] \setminus A$, if $F_A(\cdot):= \sum_{m\in A}F_m(\cdot)$, then for all $w\in \www$, such that $\nabla F_A(w)\neq 0$, $\nabla F_A(w)\notin Span\{\nabla F_m(w): m\in B\}$.
\end{lemma}
\begin{remark}
    Although Assumption \ref{ass:hetero} might sound restrictive, we only require the more relaxed property in Lemma \ref{lem:ass_hetero} to be true, and that too only for all the iterates outputted by Algorithm \ref{alg:reweight}. 
    % In general, for problems where $\www\subseteq \rr^d$ and $d\gg M$, one would expect assumption \ref{ass:hetero} to be true.\todohs{this claim is incorrect since if $F_1 =F_2$, $d\gg 2$ cannot guarantee assumption \ref{ass:hetero} to be true. }\kkp{give some example with random initialization and random updates.}
\end{remark}


% \LinesNumberedHidden{
% \begin{algorithm}[H]\caption{Defection Prediction}\label{alg:def-detect}
% \textbf{Parameters:} current point $w$, step-size $\eta$, some precision threshold $\epsilon'$\\
%     \textbf{Option I:} $S = \{m\in[M]: F_m\rb{w - \eta \cdot \ngrad{m}(w)}\leq \epsilon'\}$\\ 
%     \textbf{Option II:} $S = \{m\in[M]: F_m(w) - \eta\norm{\nabla F_m(w)}\leq \epsilon'\}$\\
%     \textbf{return} $S$ 
% \end{algorithm}}
We have the following convergence guarantee for Algorithm \ref{alg:reweight}.
\begin{theorem}\label{thm:two_agents}
   Suppose $\{F_m\}_{m\in[M]} $, satisfy Assumptions \ref{ass:cvx_smth}, \ref{ass:lip}, \ref{ass:realizable}, \ref{ass:hetero}. If we choose $w_0\notin \cup_{m\in[M]}S_m^\star$ and $\eta\leq \min\cb{\frac{\epsilon}{L}, \sqrt{\frac{\epsilon}{2H}}, \sqrt{\frac{2}{H}}, \frac{1}{MH}}$, then Algorithm~\ref{alg:reweight} will output $\hat w$ that satisfies $F(\hat w) \leq 4\epsilon$.
\end{theorem}
% \vspace{-0.5em}
According to Theorem \ref{thm:two_agents}, our proposed method can output an approximately optimal model. Note that by the design of our algorithm, we can guarantee that no agent will defect during the training process. 
Next, we provide the proof sketch of Theorem \ref{thm:two_agents}, demonstrating how our algorithm effectively avoids defection while simultaneously progressing.
% \vspace{-1em}
\begin{proof}[Proof sketch of Theorem \ref{thm:two_agents}]
% We will state some lemmas highlighting the key properties of the algorithm. Appendix \ref{app:alg} includes all the lemmas' proofs. 
First, note that to predict whether an agent defects, we look at the first-order linear lower bound on the function on each machine (see line 6). This gives a conservative estimate of whether an agent will defect if they make a personalized update. 
% because the agents' objectives are convex. 
% Since we maintain a small step size throughout, this intuitively indicates that the machine is close to defecting. 
% Moreover, this query can be implemented with a single first-order oracle call at point $w_{t-1}$ at time $t$. 
% \vspace{-0.5em}
\begin{lemma}[Predicting defections with single first-order oracle call]\label{lem:defection_detect}
    Under the same conditions of Theorem \ref{thm:two_agents}, at any time step $t$ assuming $\eta \leq \sqrt{2/H}$,
    % \vspace{-2\topsep}
    \begin{itemize}[noitemsep]
        \item if agent $m\in D$ then $F_m(w_{t-1} - \eta\ngrad{m}(w_{t-1}))\leq 3\epsilon$, and
        \item if agent $m\in ND$ then $F_m(w_{t-1}~-~\eta\ngrad{m}(w_{t-1}))~>~2\epsilon$.
    \end{itemize}
\end{lemma}
% \vspace{-0.5em}
Once we make these predictions, there are three possible cases. In case 1, some agents might defect while others will not. In case 2, no agents are predicted to defect. In case 3, all agents are predicted to defect. Since the predictions are based on the personalized update, we still need to prove if the defection might happen based on the actual update in the algorithm. We first prove that defections don't happen in case 1 and case 2 when an update is made, i.e., case 1.a and case 2.a.  
\begin{lemma}[No agent will defect in case 1.a and case 2.a]\label{lem:case1a_2a_defect}
    Under the same conditions as in Theorem \ref{thm:two_agents}. Suppose the algorithm is in case 1.a or case 2.a at any time step $t$, and no agent has defected up to time step $t$. If $\eta \leq  \sqrt{\epsilon/(2H)}$, no defection will occur once the update is made. 
\end{lemma}
% \vspace{-1em}
We also show that our algorithm makes non-zero progress on the average objective in these cases.
\begin{lemma}[Progress in case 1.a and 2.a]\label{lem:case1a_2a_progress}
    Under the same conditions as in Theorem \ref{thm:two_agents}. Suppose the algorithm is in case 1.a or 2.a at any time step $t$, and no agent has defected up to time step $t$. If $\eta \leq 1/(MH)$, then $F(w_t) < F(w_{t-1})$.
\end{lemma}
% \begin{lemma}[Progress in case 2.a]\label{lem:case2a_progress}
%     Under the same conditions as in Theorem \ref{thm:two_agents}. Suppose that the algorithm is in case 2.a at any time step $t$, and no agent has defected up to time step $t$. If $\eta \leq 1/H$, then $F(w_t) < F(w_{t-1})$.
% \end{lemma}
% \vspace{-1em}
Since the algorithm can't keep reducing the average function value ad-infinitum, the above two lemmas imply that the algorithm must stop at some point. This can happen without returning any solutions by ending up in case 0 or case 1.c. But the assumption about $w_0$ in Theorem \ref{thm:two_agents} and Assumption \ref{ass:hetero} respectively preclude running up in these cases. Thus, the algorithm can only terminate by returning a solution in cases 1.b, 2.b, 3. We show that the returned solution in these cases is good. 
\begin{lemma}[Terminating in case 1.b, 2.b, or 3 is good]\label{lem:case1b_2b_3}
    Under the same conditions as in Theorem \ref{thm:two_agents}. Suppose Algorithm~\ref{alg:reweight} terminates in case 1.b, 2.b., or 3 at time step $t$, and no agent has defected up to time step $t$. If $\eta \leq \min\cb{\sqrt{2\epsilon/H}, \epsilon/L}$, then the algorithm will output $\hat w$ that satisfies $F(\hat w) \leq 4\epsilon$.
\end{lemma}
% \vspace{-1em}
This proves the theorem. 
\end{proof}


\begin{figure}[!t]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/comparison1.pdf}
         \caption{
         Both algorithms use $\eta=0.001$ and $\epsilon=0.4$.}
         \label{fig:comparison_1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/comparison2.pdf}
         \caption{
         $\epsilon=0.5$, $\eta_{\textsc{FedAvg}}=2e^{-5}$, $\eta_{\textsc{ADA-GD}}=2e^{-4}$.}
         \label{fig:comparison_2}
     \end{subfigure}
        \caption{We study the performance of our method and federated averaging (local SGD) for binary classification on two classes of CIFAR-10 \cite{krizhevsky2009learning} with two agents. The data heterogeneity $q=0.9$ and local update step $K=1$ for both experiments. Figure \ref{fig:comparison_1} shows that Local-SGD results in agent defection around the $130$-th iteration, leading to a considerable decay in the accuracy of the final model. In sharp contrast, our proposed method effectively eliminates defection, enabling the continuous improvement of the model throughout the training process. In Figure \ref{fig:comparison_2}, we study the performance of both algorithms with the largest step size such that no agents will defect. We observe that \textsc{ADA-GD} can avoid defection even when employing a considerably larger step size than local SGD. As a result, this enables us to attain a significantly improved final model. These results support our theoretical findings and validate the effectiveness of our method.}
        \label{fig:our_algorithm}
        % \vspace{-1em}
\end{figure}

% \begin{proof}[Proof of Theorem \ref{thm:two_agents}]
% We will show that algorithm \ref{alg:reweight} with a small enough step-size sequence,
% \vspace{-\topsep}
% \begin{enumerate}[noitemsep]
%     \item will terminate in either case 1.b, case 2.b, or case 3 if it terminates, 
%     \item will not cause any agent to defect, and
%     \item will output a model $\hat{w}$ which is approximately optimal.
% \end{enumerate}
%  The first property can be seen by observing the procedure of the algorithm. First, assume the algorithm terminates (we show this for property 3. below). Since we assume $w_0\notin \cup_{m\in[M]}S_m^\star$, the algorithm doesn't terminate in case 0. Furthermore, due to assumption \ref{ass:hetero} and lemma \ref{lem:ass_hetero}), the algorithm will never terminate in case 1.c. Thus the algorithm can only terminate while returning $\hat{w}$ in cases 1.b, 2.b, or 3.

% Now to see the second property, note that defections can only happen if (i) the algorithm runs into case 1.a or 2.a, (ii) it makes the corresponding update, and (iii) the agent chooses to defect after seeing the updated model. We show no agent defects in case 1.a (see lemma \ref{lem:case1a__2a_defect}). This is because we create our update direction in case 1.a so that for all agents in $D$, the update is orthogonal to their current gradient, and thus they don't reduce their objective value. And for all agents in $ND$, they do make progress, but we control the step size so that they don't make \textit{``too much progress"}. Thus no agent defects in case 1.a. Similarly, in case 2.a we avoid defections by ensuring the step size is small enough (see lemma \ref{lem:case1a_2a_defect}). 

% Finally, to show the third property, we note that the model is returned in only three cases, cases 1.b, cases 2.b, and 3. We can show that in all these cases, the model has final performance on the average objective, which is $\ooo(\epsilon)$ (see lemmas \ref{lem:case1b}, \ref{lem:case2b} and \ref{lem:case3} respectively). But this doesn't prove the property as what ensures the algorithm will indeed terminate. For instance, it could converge to a model without moving to the termination cases or even oscillate between a few models without converging forever. To prove that the algorithm terminates, it is enough\todohs{possibly always stay in case 1.a and 2.a, $F(w_t)$ is converging but never terminate.} to show that the algorithm makes non-zero progress on the average objective every time it is in case 1.a and case 2.a. We precisely show this in lemmas \ref{lem:case1a_progress} and \ref{lem:case2a_progress} respectively. To show this in lemma \ref{lem:case1a_progress}, we rely on the specific construction of the update and assumption \ref{ass:hetero}. While to show this in lemma \ref{lem:case2a_progress}, we need to pick the appropriate step size (to avoid defections) as we are already moving in the steepest descent direction.

% Thus combining the three properties, we can conclude that the algorithm outputs a good model and avoids defections. This finishes the proof.  
% \end{proof}


























==> src/alg.tex <==
% \todohs{maybe move the current remark to motivate the idea of providing a bad model to agents with low loss}
% \begin{remark}
%     Notice that the defection depends on the loss function and the synchronized model provided by the server.
%     Suppose that the loss $f(w;(x,y)) = -(2y-1)w^\top x$ is a linear function. Then the local update on each machine is an accumulation of local data which does not depend on the given model! 
%     Thus the server can cheat by sending each agent a fake model $w^m_{rK} =\bZero$ for $rK<T$ and no agent will defect if $\bZero$ is not a good model.
%     Once the server collects enough data, it outputs the true synchronized model in the final round.
% \end{remark}
% \todohs{Add a brief description on the potential method as we discussed}

\begin{algorithm}[H]\caption{Adaptive Defection-aware Aggregation for Gradient Descent (\textsc{ADA-GD})}\label{alg:reweight}
\textbf{Parameters:} step size $\eta$, initialization $w_{0}$\\
    % Initialize at $w_{0}$\\
    % \If{$\exists m\in[M], \text{ s.t. }F_m(w_0)\leq \epsilon$}{
    % STOP \Comment{Case 0\hs{to remove}}
    % } 
    \For{$t=1,2,\ldots$}{
    Compute $\nabla F_m(w_{t-1})$ for all $m\in[M]$\\
    \textbf{Predict defecting agents:} $D = \{m\in[M]: F_m(w_{t-1}) - \eta\norm{\nabla F_m(w_{t-1})}\leq 2\epsilon\}$\label{alg-step:defecting}\\ 
    \textbf{Predict non-defecting agents:} $ND = [M]\setminus D$\label{alg-step:non-defecting}\\
    \If{Both $D$ and $ND$ are non-empty}{
    Compute $\nabla F_{ND}(w_{t-1}) = \sum_{m\in ND}\nabla F_m(w_{t-1})$\\
    Let $P = Span\{\nabla F_n(w_{t-1}): n\in D\}^\perp$\\
    % \If{$\norm{\Pi_P\rb{\nabla F_{ND}(w_{t-1})}}\neq 0$}
    {
    Project $\nabla F_{ND}(w_{t-1})$ and normalize $\ngrad{ND}(w_{t-1}) = \frac{\Pi_P\rb{\nabla F_{ND}(w_{t-1})}}{\norm{\Pi_P\rb{\nabla F_{ND}(w_{t-1})}}}$\\
    $g_t = -\min\cb{\norm{\Pi_P\rb{\nabla F_{ND}(w_{t-1})}}, 1}\cdot\ngrad{ND}(w_{t-1})$\Comment{Case 1}\label{alg-step:some-defect}\\
    }
    % \Else{
    % \If{$\nabla F_{ND}(w_{t-1})=0$}{
    % \Return $\hat{w} = w_{t-1}$ \Comment{Case 1.b\hs{tr}}\\
    % }
    % \Else{
    % STOP \Comment{Case 1.c\hs{tr}}\\
    % }
    % }
    }
    \If{$D$ is empty}{
    % \If{$\nabla F(w_{t-1})\neq 0$}
    {
    $g_t = -\min\{\norm{\nabla F(w_{t-1})}, 1\}\cdot\frac{\nabla F(w_{t-1})}{\norm{\nabla F(w_{t-1})}}$ \Comment{Case 2}\label{alg-step:no-defect}\\
    }
    % \Else{
    % \Return $\hat{w} = w_{t-1}$ \Comment{Case 2.b\hs{to remove}}
    % }
    }
    %\\
    \If{$ND$ is empty }{
    \Return $\hat{w}= w_{t-1}$ \Comment{Case 3}\label{alg-step:all-defect}
    }
    $w_t = w_{t-1} + \eta g_t$
    }  
\end{algorithm}

In this section, we will introduce algorithm \ref{alg:reweight}. Before we discuss our algorithm, let's recall the definition of the orthogonal complement of a subspace. 
\begin{definition}[Orthogonal Complement]
    Let $V$ be a vector space with an inner-product $\inner{\cdot}{\cdot}$. For any subspace $U$ of $V$, we define the orthogonal complement as $U^\perp := \{v\in V: \inner{v}{u} = 0,\ \forall u\in U\}$. We also define the projection operator onto a subspace $U$ by $\Pi_{U}:V\to U$. 
\end{definition}
Our algorithm \textsc{ADA-GD} is stated in Algorithm \ref{alg:reweight}. At our method's core is an adaptive aggregation approach for the gradients received from agents, which disincentivizes participating agents' defection during the training. 
However, disincentivizing defection is impossible if two agents are very ``similar''. Consider the example of $F_1(w) = \norm{w}^2$ and $F_2 = \epsilon\norm{w}^2$. Whenever we reach some $w_t$ with $\norm{w_t}^2\in (\epsilon, 1]$ (otherwise, we have to jump from some $w_{t-1}$ with $\norm{w_{t-1}}^2 >1$ to some $w_{t}$ with $\norm{w_{t}}^2 \leq \epsilon$), agent $2$ will defect. 
Therefore, we must introduce some heterogeneity assumption implying that the functions are \textit{``dissimilar enough''}. 
\begin{assumption}[Minimal Heterogeneity]\label{ass:hetero}
    Consider differentiable functions $\{F_m:\rr^d\to \rr\}$. Then for all $w\in \www\setminus \www^\star$, all non-zero vectors in $\{\nabla F_m(w): m\in[M]\}$ are linearly independent.
\end{assumption}

\begin{remark}
% We actually require this linear independence property to hold only for all the iterates outputted by Algorithm \ref{alg:reweight}. 
To justify the necessity of this linear independence assumption, one may argue that in the above simple example, the defection is benign. We provide a more complicated example where linear dependence leads to harmful defections in Figure~\ref{fig:defection_example}.
\end{remark}





Under Assumptions \ref{ass:cvx_smth}, \ref{ass:lip}, \ref{ass:realizable}, \ref{ass:hetero}, we show that our algorithm is legal (i.e., any denominator in Algorithm~\ref{alg:reweight} is non-zero) and converges to an approximately optimal model.
\begin{theorem}\label{thm:two_agents}
   Suppose $\{F_m\}_{m\in[M]} $, satisfy Assumptions \ref{ass:cvx_smth}, \ref{ass:lip}, \ref{ass:realizable}, \ref{ass:hetero}. If we choose $w_0\notin \cup_{m\in[M]}S_m^\star$ and $\eta\leq \min\cb{\frac{\epsilon}{L}, \sqrt{\frac{\epsilon}{2H}}, \sqrt{\frac{2}{H}}, \frac{1}{MH}}$, then no agents will defect and Algorithm~\ref{alg:reweight} will output $\hat w$ that satisfies $F(\hat w) \leq 4\epsilon$.
\end{theorem}


Now we outline the high-level ideas behind Algorithm~\ref{alg:reweight}.
Intuitively, an agent is close to defection if a direction $u$ exists such that she would defect after receiving $w_{t-1}-\eta u$.
Hence, the server has to carefully tune the update direction to avoid the defection of this agent.



Suppose no agent has defected upon receiving $w_{t-1}$. Then, the server will receive the first-order information $\ooo_m(w_{t-1})$ from all agents and determine a direction to update $w_{t-1}$ to $w_t$.
In Algorithm~\ref{alg:reweight}, the server first predicts which agents are close to defection through a linear approximation (see line \ref{alg-step:defecting}) and calls them `defecting' agents (although these agents might not defect because of the slack in the precision in line \ref{alg-step:defecting}).
% check if each agent $m$ is close to defection through the linear approximation of the agent loss if we set update $ w_{t-1}$ in the direction of $-\nabla F_m(w_t)$.
% Since $\nabla F_m(w_{t-1})$ is the steepest decreasing direction for $F_m(w_{t-1})$, this linear approximation provides a lower bound of $F(w_t)$ no matter what direction we update.
% Therefore, here defecting agents are agents who have chance to defect after receiving $w_t$ while non-defecting agents will certainly not defect after receiving $w_t$.
If all agents are `defecting' (case 3), the server will output the current model $w_{t-1}$ as the final model (see line~\ref{alg-step:all-defect}). The output model is approximately optimal since each agent has a small $F_m(w_{t-1})$ when they are `defecting'.
If no agent is `defecting' (case 2), the server is certain that all agents will not defect after the update and thus will update in the steepest descending direction, i.e., the gradient of the average loss $\nabla F(w_{t-1})$ (see line~\ref{alg-step:no-defect}).
If there exist both `defecting' and `non-defecting' agents (case 1), the server will aggregate
% \lw{how about simplify as "If there exist both `defecting' and `non-defecting' agents (case 1), the server will aggregate ..." }It becomes complicated when there exist both `defecting' and `non-defecting' agents (case 1). To guarantee that `defecting' agents will not defect upon receiving $w_t$, the server will aggregate
the gradients from non-defecting agents and project them to the orthogonal complement of the space spanned by the gradients of the `defecting' agents to guarantee that `defecting' agents will not defect. Then, the server will update the current model using the normalized projected gradients (see line~\ref{alg-step:some-defect}).
By induction, we can show that no agents will defect. Furthermore, we can prove that we will make positive progress in decreasing the average loss at each round, and as a result, our algorithm will ultimately converge to an approximately optimal model. Our analysis is inherently case-based, making it difficult to replicate a simple distributed gradient descent analysis that proceeds by showing that we move in a descent direction at each iteration. Consequently, offering a convergence rate poses a significant challenge and remains an open question.


Note that Algorithm \ref{alg:reweight} fits in the class of ICFO algorithms specified in Section~\ref{sec:setup}, as orthogonalization and normalization return an output in the linear span of the machines' gradients. In Figure \ref{fig:our_algorithm}, we compare \textsc{ADA-GD} against \textsc{FedAvg}, demonstrating the benefit of adaptive aggregation. 



% If it is certain that no agent will defect, the server will normalize the uniform aggregated gradient and use it to update the current model (see line~\ref{alg-step:no-defect}). 
% If it is predicted that all the agents defect, the server will output the current model as the final model (see line~\ref{alg-step:all-defect}). 
% Suppose there exist both defecting and non-defecting agents. In that case, the server will aggregate the gradients from non-defecting agents and project them to the orthogonal complement of the space spanned by the gradients of the defecting agents. Then, the server will update the current model using the normalized projected gradients (see line 8 to line 18). 
% This is almost without loss of generality as for applications such as cross-device federated learning, we want to pick a representative and diverse set of devices that are not replaceable by other devices in the selection.




\begin{figure}[!t]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{fig/comparison1.pdf}
         \caption{
         Both algorithms use $\eta=0.001$ and $\epsilon=0.4$.}
         \label{fig:comparison_1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=0.8\textwidth]{fig/comparison2.pdf}
         \caption{
         $\epsilon=0.5$, $\eta_{\textsc{LSGD}}=2e^{-5}$, $\eta_{\textsc{ADA-GD}}=2e^{-4}$.}
         \label{fig:comparison_2}
     \end{subfigure}
        \caption{We study the performance of our method and federated averaging (local SGD) for binary classification on two classes of CIFAR-10 \citep{krizhevsky2009learning} with two agents. The data heterogeneity $q=0.9$ and local update step $K=1$ for both experiments. Figure \ref{fig:comparison_1} shows that Local SGD results in agent defection around the $130$-th iteration, leading to a considerable decay in the accuracy of the final model. In sharp contrast, our proposed method effectively eliminates defection, enabling the continuous improvement of the model throughout the training process. Remark that it's unfair to compare the highest accuracy of Local SGD with our method as Local SGD is not defection aware and could not simply stop at the highest point. In Figure \ref{fig:comparison_2}, we study the performance of both algorithms with the largest step size such that no agents will defect. We observe that \textsc{ADA-GD} can avoid defection even when employing a considerably larger step size than Local SGD. As a result, this enables us to attain a significantly improved final model. These results support our theoretical findings and validate the effectiveness of our method.}
        \label{fig:our_algorithm}
        \vspace{-1em}
\end{figure}

% \begin{proof}[Proof of Theorem \ref{thm:two_agents}]
% We will show that algorithm \ref{alg:reweight} with a small enough step-size sequence,
% \vspace{-\topsep}
% \begin{enumerate}[noitemsep]
%     \item will terminate in either case 1.b, case 2.b, or case 3 if it terminates, 
%     \item will not cause any agent to defect, and
%     \item will output a model $\hat{w}$ which is approximately optimal.
% \end{enumerate}
%  The first property can be seen by observing the procedure of the algorithm. First, assume the algorithm terminates (we show this for property 3. below). Since we assume $w_0\notin \cup_{m\in[M]}S_m^\star$, the algorithm doesn't terminate in case 0. Furthermore, due to assumption \ref{ass:hetero} and lemma \ref{lem:ass_hetero}), the algorithm will never terminate in case 1.c. Thus the algorithm can only terminate while returning $\hat{w}$ in cases 1.b, 2.b, or 3.

% Now to see the second property, note that defections can only happen if (i) the algorithm runs into case 1.a or 2.a, (ii) it makes the corresponding update, and (iii) the agent chooses to defect after seeing the updated model. We show no agent defects in case 1.a (see lemma \ref{lem:case1a__2a_defect}). This is because we create our update direction in case 1.a so that for all agents in $D$, the update is orthogonal to their current gradient, and thus they don't reduce their objective value. And for all agents in $ND$, they do make progress, but we control the step size so that they don't make \textit{``too much progress"}. Thus no agent defects in case 1.a. Similarly, in case 2.a we avoid defections by ensuring the step size is small enough (see lemma \ref{lem:case1a_2a_defect}). 

% Finally, to show the third property, we note that the model is returned in only three cases, cases 1.b, cases 2.b, and 3. We can show that in all these cases, the model has final performance on the average objective, which is $\ooo(\epsilon)$ (see lemmas \ref{lem:case1b}, \ref{lem:case2b} and \ref{lem:case3} respectively). But this doesn't prove the property as what ensures the algorithm will indeed terminate. For instance, it could converge to a model without moving to the termination cases or even oscillate between a few models without converging forever. To prove that the algorithm terminates, it is enough\todohs{possibly always stay in case 1.a and 2.a, $F(w_t)$ is converging but never terminate.} to show that the algorithm makes non-zero progress on the average objective every time it is in case 1.a and case 2.a. We precisely show this in lemmas \ref{lem:case1a_progress} and \ref{lem:case2a_progress} respectively. To show this in lemma \ref{lem:case1a_progress}, we rely on the specific construction of the update and assumption \ref{ass:hetero}. While to show this in lemma \ref{lem:case2a_progress}, we need to pick the appropriate step size (to avoid defections) as we are already moving in the steepest descent direction.

% Thus combining the three properties, we can conclude that the algorithm outputs a good model and avoids defections. This finishes the proof.  
% \end{proof}


























==> src/alg_proof-backup.tex <==
\subsection{Proof of theorem \ref{thm:two_agents}}
\begin{proof}[Proof of Theorem \ref{thm:two_agents}]
We will show that algorithm \ref{alg:reweight} with a small enough step-size sequence,
\vspace{-\topsep}
\begin{enumerate}[noitemsep]
    \item will terminate in either case 1.b, case 2.b, or case 3 if it terminates, 
    \item will not cause any agent to defect, and
    \item will output a model $\hat{w}$ which is approximately optimal.
\end{enumerate}
 The first property can be seen by observing the procedure of the algorithm. First, assume the algorithm terminates (we show this for property 3. below). Since we assume $w_0\notin \cup_{m\in[M]}S_m^\star$, the algorithm doesn't terminate in case 0. Furthermore, due to assumption \ref{ass:hetero} and lemma \ref{lem:ass_hetero}), the algorithm will never terminate in case 1.c. Thus the algorithm can only terminate while returning $\hat{w}$ in cases 1.b, 2.b, or 3.

Now to see the second property, note that defections can only happen if (i) the algorithm runs into case 1.a or 2.a, (ii) it makes the corresponding update, and (iii) the agent chooses to defect after seeing the updated model. We show no agent defects in case 1.a (see lemma \ref{lem:case1a_2a_defect}). This is because we create our update direction in case 1.a so that for all agents in $D$, the update is orthogonal to their current gradient, and thus they don't reduce their objective value. And for all agents in $ND$, they do make progress, but we control the step size so that they don't make \textit{``too much progress"}. Thus no agent defects in case 1.a. Similarly, in case 2.a we avoid defections by ensuring the step size is small enough (see lemma \ref{lem:case1a_2a_defect}). 

Finally, to show the third property, we note that the model is returned in only three cases, cases 1.b, cases 2.b, and 3. We can show that in all these cases, the model has the final performance on the average objective, which is $\ooo(\epsilon)$ (see lemma \ref{lem:case1b_2b_3}). But this doesn't prove the property as what ensures the algorithm will indeed terminate. For instance, it could converge to a model without moving to the termination cases or even oscillate between a few models without converging forever. To prove that the algorithm terminates, it is enough to show that the algorithm makes non-zero progress on the average objective every time it is in case 1.a and case 2.a. We precisely show this in lemma \ref{lem:case1a_2a_progress}. To show this in case 1a, we rely on the specific construction of the update and assumption \ref{ass:hetero}. While to show this in case 2a, we need to pick the appropriate step size (to avoid defections) as we are already moving in the steepest descent direction.

Thus combining the three properties, we can conclude that the algorithm outputs a good model and avoids defections. This finishes the proof.  
\end{proof}

\subsection{Proof of lemma \ref{lem:ass_hetero}}

\begin{proof}
    Consider some point $w\in\www\setminus \www^\star$ and let the non-zero gradients on the agents be linearly independent at that point. If possible, let the above property be violated, then we have at least one $A\subseteq [M]$ such that $\nabla F_A(w) \in Span\{\nabla F_m(w): m\in B\}$ and $\nabla F_A\neq 0$. In particular there are coefficients $\{\gamma_n\in \rr\}_{n\in B}$ (not all zero) such that,  
    \begin{align*}
        &\sum_{m\in A}\nabla F_m(w) = \sum_{n\in B}\gamma_n \nabla F_n(w),\\
        &\Leftrightarrow \sum_{m\in A}\nabla F_m(w)  + \sum_{n\in B}(-\gamma_n) \nabla F_n(w) = 0,
    \end{align*}
    This implies that the gradients are linearly dependent (note that not all gradients can be zero as then $w$ would be in $\www^\star$), which is a contradiction.
    % Now for the other direction let's assume that the property is true for some $w\in\www$. Then we know that for all $m\in[M]$, $\nabla F_m(w)\notin Span\{\nabla F_n(w): n\in[M]\setminus\{m\}\}$. 
    % % In particular assuming this implies that there are no coefficients $\{\gamma_n\in\rr\}_{n\in[M]\setminus \{m\}}$ such that,
    % % \begin{align*}
    % %     \nabla F_m(w) \in \sum_{n\in[M]\setminus \{m\}}\gamma_n \nabla F_n(w). 
    % % \end{align*}
    % Let $m$ above be such that $\nabla F_m(w)\neq 0$. Now assume if possible that the gradients on the machines are linear dependent. Then there exist coefficients $\{\gamma_n\in\rr\}_{n\in[M]}$ such that,
\end{proof}

\subsection{Proof of lemma \ref{lem:defection_detect}}
\begin{proof}
    Let's say we are at time step $t$. Assume $m\in D$ and note that the smoothness of function $F_m$ implies that,
    \begin{align*}
        F_m(w_{t-1} - \eta_t\ngrad{m}(w_{t-1})) &\leq F_m(w_{t-1}) + \inner{\nabla F_m(w_{t-1})}{-\eta_t\ngrad{m}(w_{t-1})} + \frac{H}{2}\norm{\eta_t\ngrad{m}(w_{t-1})}^2,\\ 
        &= F_m(w_{t-1}) -\eta_t\norm{\nabla F_m(w_{t-1})} + \frac{H\eta_t^2}{2},\\
        &\leq^{(m\in D)} 2\epsilon + \frac{H\eta_t^2}{2},\\
        &\leq 3\epsilon,
    \end{align*}
    where we used that $\eta_t \leq \sqrt{\frac{2}{H}}$. Now assume $m\in ND$ and note using convexity of $F_m$ that,
    \begin{align*}
        F_m(w_{t-1} - \eta_t\ngrad{m}(w_{t-1})) &\geq F_m(w_{t-1}) + \inner{\nabla F_m(w_{t-1})}{-\eta_t\ngrad{m}(w_{t-1})},\\ 
        &= F_m(w_{t-1}) -\eta_t\norm{\nabla F_m(w_{t-1})},\\
        &>^{(m\in ND)} 2\epsilon.
    \end{align*}
    This proves the lemma.
\end{proof}

\subsection{Proof of Lemma \ref{lem:case1a_2a_defect}}
\begin{proof}
    First, assume we are in case 1.a at time $t$. Let's first show that we don't make any agent $m\in D$ defect,
\begin{align*}
    F_m(w_t) &\geq F_{m}(w_{t-1}) + \inner{\nabla F_{m}(w_{t-1})}{g_t},\\
    &= F_{m}(w_{t-1}),\\
    &> \epsilon,
\end{align*}
as $g_t\perp \nabla F_{m}(w_{t-1})$ for all $m\in D$ by design and no agent defected up to time $t$. For any non-defecting agent $m\in ND$ we have,
    \begin{align*}
        &F_{m}(w_{t-1} + \eta_t g_t)-F_{m}(w_{t-1} - \eta_t \ngrad{m}(w_{t-1})) \\
        &\geq^{\text{(convexity)}}\inner{\nabla F_{m}(w_{t-1} - \eta_t \ngrad{m}(w_{t-1}))}{\eta_t(g_t +\ngrad{m}(w_{t-1}))},\\
        &= \inner{\nabla F_{m}(w_{t-1} - \eta_t \ngrad{m}(w_{t-1})) -\nabla F_{m}(w_{t-1}) + \nabla F_{m}(w_{t-1})}{\eta_t(g_t +\ngrad{m}(w_{t-1}))},\\
        &\geq^{\text{(C.S. inequality)}} \inner{\nabla F_{m}(w_{t-1} )}{\eta_t(g_t +\ngrad{m}(w_{t-1}))}\\
        &\qquad - \norm{\nabla F_{m}(w_{t-1}) - \nabla F_{m}(w_{t-1} - \eta_t \ngrad{m}(w_{t-1}))}\cdot \norm{\eta_t(g_t +\ngrad{m}(w_{t-1}))},\\
        &\geq^{\text{(Ass. \ref{ass:cvx_smth})}} \inner{\nabla F_{m}(w_{t-1} )}{\eta_t(g_t +\ngrad{m}(w_{t-1}))} - \eta_t^2 H\norm{\ngrad{m}(w_{t-1})}\cdot \norm{g_t +\ngrad{m}(w_{t-1})},\\
        &\geq^{\text{(normalized gradients)}} \inner{\nabla F_{m}(w_{t-1} )}{\eta_t(g_t +\ngrad{m}(w_{t-1}))} - 2\eta_t^2H,\\
        &= \eta_t\norm{\nabla F_{m}(w_{t-1} )}\rb{1 + \inner{\ngrad{m}(w_{t-1})}{g_t}} - 2\eta_t^2H,\\
        &\geq - 2\eta_t^2H,
    \end{align*}
    Re-arranging this gives the following,
    \begin{align*}
        F_{m}(w_{t-1} + \eta_t g_t) &\geq F_{m}(w_{t-1} - \eta_t \ngrad{m}(w_{t-1})) - 2\eta_t^2H\\
        &>^{(\text{lemma \ref{lem:defection_detect}})} 2\epsilon - 2\eta_t^2H,\\
        &\geq \epsilon, 
    \end{align*}
    where we assume that $\eta_t \leq \sqrt{\frac{\epsilon}{2H}}$.  

    Now assume instead we are in case 2.a at time $t$. For agent $m\in[M]$ we have,
    \begin{align*}
        &F_{m}(w_{t-1} + \eta_t g_t)-F_{m}(w_{t-1} - \eta_t \ngrad{m}(w_{t-1})) \\
        &\geq^{\text{(convexity)}}\inner{\nabla F_{m}(w_{t-1} - \eta_t \ngrad{m}(w_{t-1}))}{\eta_t(g_t +\ngrad{m}(w_{t-1}))},\\
        &= \inner{\nabla F_{m}(w_{t-1} - \eta_t \ngrad{m}(w_{t-1})) -\nabla F_{m}(w_{t-1}) + \nabla F_{m}(w_{t-1})}{\eta_t(g_t +\ngrad{m}(w_{t-1}))},\\
        &\geq^{\text{(C.S. inequality)}} \inner{\nabla F_{m}(w_{t-1} )}{\eta_t(g_t +\ngrad{m}(w_{t-1}))}\\
        &\qquad - \norm{\nabla F_{m}(w_{t-1}) - \nabla F_{m}(w_{t-1} - \eta_t \ngrad{m}(w_{t-1}))}\cdot \norm{\eta_t(g_t +\ngrad{m}(w_{t-1}))},\\
        &\geq^{\text{(Ass. \ref{ass:cvx_smth})}} \inner{\nabla F_{m}(w_{t-1} )}{\eta_t(g_t +\ngrad{m}(w_{t-1}))} - \eta_t^2 H\norm{\ngrad{m}(w_{t-1})}\cdot \norm{g_t +\ngrad{m}(w_{t-1})},\\
        &\geq \inner{\nabla F_{m}(w_{t-1} )}{\eta_t(g_t +\ngrad{m}(w_{t-1}))} - 2\eta_t^2H,\\
        &= \eta_t\norm{\nabla F_{m}(w_{t-1})}\rb{1 + \inner{\ngrad{m}(w_{t-1})}{g_t}} - 2\eta_t^2H,\\
        &\geq - 2\eta_t^2H.
    \end{align*}
    Choosing $\eta_t \leq \sqrt{\frac{\epsilon}{2H}}$ ensures that, 
    \begin{align*}
        F_{m}(w_{t}) >^{\text{(lemma \ref{lem:defection_detect})}} 2\epsilon - \epsilon = \epsilon,
    \end{align*}
    and thus agent $m$ doesn't defect.
\end{proof}

\subsection{Proof of Lemma \ref{lem:case1a_2a_progress}}
\begin{proof}
We first assume we make an update in \textbf{case 1a}. First, using the smoothness assumption and then using the fact that $g_t$ is orthogonal to the gradients of all the agents in $D$, we get
    \begin{align*}
        F(w_t) &= F(w_{t-1}+\eta g_t),\\
        &\leq^{\text{(ass. \ref{ass:cvx_smth})}} F(w_{t-1}) + \eta \inner{\frac{\sum_{m\in D}\nabla F_{m}(w_{t-1}) + \nabla F_{ND}(w_{t-1})}{M}}{g_t} + \frac{H\eta^2}{2} \norm{g_t}^2,\\
        &\leq F(w_{t-1}) -\frac{\eta}{M} \inner{\nabla F_{ND}(w_{t-1})}{g_t} +\frac{H\eta^2}{2} \norm{g_t}^2,\\
        % &= F(w_{t-1}) -\frac{\eta}{M} \norm{\nabla F_{ND}(w_{t-1})} + \frac{H\eta^2}{2},\\
        % &\leq F(w_{t-1}) -\frac{\eta}{2M} \norm{\nabla F_{ND}(w_{t-1})},\\
        % &< F(w_{t-1}),
    \end{align*}
    Now we will consider two cases. In the first case, assume $\norm{\nabla F_{ND}(w_{t-1})}< 1$. Then we get that,
    \begin{align*}
        F(w_t)&\leq F(w_{t-1}) -\frac{\eta}{M} \inner{\nabla F_{ND}(w_{t-1})}{\nabla F_{ND}(w_{t-1})} +\frac{H\eta^2}{2} \norm{\nabla F_{ND}(w_{t-1})}^2,\\
        &\leq F(w_{t-1}) -\frac{\eta}{M}\norm{\nabla F_{ND}(w_{t-1})}^2 +\frac{H\eta^2}{2} \norm{\nabla F_{ND}(w_{t-1})}^2,\\
        &\leq F(w_{t-1}) -\frac{\eta_t}{2M}\norm{\nabla F_{ND}(w_{t-1})}^2,
    \end{align*}
    where we assume $\eta_t \leq \frac{1}{M H}$. Since in case 1.a $\norm{\nabla F_{ND}(w_{t-1})}\neq 0$, we will probably make progress on the average objective. In the second case, assume $\norm{\nabla F_{ND}(w_{t-1})}\geq 1$. Then we will get that,
    \begin{align*}
        F(w_t)&\leq F(w_{t-1}) -\frac{\eta_t}{M} \norm{\nabla F_{ND}(w_{t-1})} + \frac{H\eta_t^2}{2},\\
        &\leq F(w_{t-1}) -\frac{\eta_t}{M} +\frac{H\eta_t^2}{2},\\
        &\leq F(w_{t-1}) -\frac{\eta_t}{2M},
    \end{align*}
    where we assume $\eta_t \leq \frac{1}{M H}$. This finishes the proof. 


    Next we assume we make an update in \textbf{case 2a}. Note that using smoothness,
    \begin{align*}
        F(w_{t}) &= F(w_{t-1} + \eta_t g_t ),\\
        &\leq F(w_{t-1}) +\eta_t \inner{\nabla F(w_{t-1})}{g_t} + \frac{H\eta_t^2}{2}\norm{g_t}^2.
    \end{align*}
    Let's first assume $\norm{\nabla F(w_{t-1})}\geq 1$. Using the definition of $g_t$ we get,
    \begin{align*}
        F(w_{t}) &\leq F(w_{t-1}) -\eta_t \inner{\nabla F(w_{t-1})}{\frac{\nabla F(w_{t-1})}{\norm{\nabla F(w_{t-1})}}} + \frac{H\eta_t^2}{2}\norm{g_t}^2,\\
        &= F(w_{t-1}) -\eta_t \norm{\nabla F(w_{t-1})} + \frac{H\eta_t^2}{2},\\
        &\leq F(w_{t-1}) -\eta_t + \frac{H\eta_t^2}{2},\\
        &\leq F(w_{t-1}) -\frac{\eta_t}{2},  
    \end{align*}
    where we assume $\eta_t \leq \frac{1}{H}$. Now let's consider the case when $\norm{\nabla F(w_{t-1})}< 1$.
    \begin{align*}
        F(w_{t}) &\leq F(w_{t-1}) -\eta_t \inner{\nabla F(w_{t-1})}{\nabla F(w_{t-1})} + \frac{H\eta_t^2}{2}\norm{\nabla F(w_{t-1})}^2,\\
        &= F(w_{t-1}) -\eta_t \norm{\nabla F(w_{t-1})}^2 + \frac{H\eta_t^2}{2}\norm{\nabla F(w_{t-1})}^2,\\
        &\leq F(w_{t-1}) -\frac{\eta_t}{2}\norm{\nabla F(w_{t-1})}^2,  
    \end{align*}
    where we assume $\eta_t \leq \frac{1}{H}$. Note that $\norm{\nabla F(w_{t-1})}\neq 0$ in this case, which means the algorithm makes non-zero progress on the average objective.
\end{proof}

\subsection{Proof of Lemma \ref{lem:case1b_2b_3}}
\begin{proof}
    Consider \textbf{case 1b}. First, note that the outputted model is already good in this case for $F_{ND}$, as $\nabla F_{ND}(w_{t-1}) = 0$. This implies that $F_{ND}(w_{t-1}) = F_{ND}(w^\star)$ for $w^\star\in \www^\star$ (see case 2b). This means we can write the following for the average objective, 
    \begin{align*}
        F(w_{t-1}) &= \frac{F_{ND}(w_{t-1}) + \sum_{m\in D}F_m(w_{t-1})}{M},\\ 
        &= \frac{\sum_{m\in D}F_m(w_{t-1})}{M}.
    \end{align*}
    Now note the following for the defecting machines using smoothness (assumption \ref{ass:cvx_smth}). For all $m\in D$ we have,
    \begin{align*}
        F_m(w_{t-1}) &\leq F_m(w_{t-1} - \eta_t \ngrad{m}(w_{t-1})) -\eta_t \inner{\nabla F_m(w_{t-1})}{\ngrad{m}(w_{t-1})} + \frac{H\eta_t^2}{2}\norm{\ngrad{m}(w_{t-1})}^2,\\ 
        &\leq 2\epsilon -\eta_t\norm{\nabla F_m(w_{t-1})} + \frac{H\eta_t^2}{2},\\
        &\leq 2\epsilon + \frac{H\eta_t^2}{2}
        \leq 3\epsilon,
    \end{align*}
    where we assumed $\eta_t\leq \sqrt{\frac{2\epsilon}{H}}$. Thus we have for the average objective,
    \begin{align*}
        F(w_{t-1}) &= \frac{\sum_{m\in D}F_m(w_{t-1})}{M},\\ 
        &\leq \frac{3\epsilon |D|}{M},\\ 
        &\leq 3\epsilon,
    \end{align*}
    which proves the claim.


    Next, consider \textbf{case 2b}. Let's say that Algorithm~\ref{alg:reweight} terminates in Case 2.b at time $t$, then $\hat{w}$ is a stationary point of $F$. Since $F$ is convex, $\hat{w}$ must be a global minimum of $F$. In particular, because of our realizability assumption, there is at least one shared optimizer across all the machines. Let's say this minimizer is $w^\star$, then since all the machines are minimized at $w^\star$, for all $m\in[M]$, we must have $F_m(\hat{w}) \geq F_m(w^\star)$. Let's assume there exists machine $n\in[M]$ such that $F_n(\hat{w}) > F_n(w^\star)$, this would imply that 
    \begin{align*}
     F(w^\star) &\geq F(\hat{w}),\\ 
    &= \frac{1}{M}\sum_{m\in[M]}F_m(\hat{w}),\\
    &\geq \frac{1}{M}\sum_{m\neq n}F_m(w^\star) + \frac{F_n(\hat{w})}{M},\\
    &> \frac{1}{M}\sum_{m\neq n}F_m(w^\star) + \frac{F_n(w^\star)}{M},\\
    &= F(w^\star),
    \end{align*}
    which is a contradiction. Hence all the machines must be simultaneously minimized at $w^\star$. This proves the claim.


    Finally, consider \textbf{case 3}. Let's say that Algorithm~\ref{alg:reweight} terminates in Case 3 at time $t$ then we have for all $m \in D = [M]$,
\begin{align*}
    3\epsilon &\geq^{(\text{Lemma \ref{lem:defection_detect}})} F_{m}(w_{t-1} - \eta_t \ngrad{m}(w_{t-1})),\\ 
    &\geq^{(\text{Convexity})} F_{m}(w_{t-1}) + \inner{\nabla F_{m}(w_{t-1})}{-\eta_t\ngrad{m}(w_{t-1})},\\
    &= F_{m}(w_{t-1}) + \inner{\nabla F_{m}(w_{t-1})}{-\eta_t \frac{\nabla F_{m}(w_{t-1})}{\norm{\nabla F_{m}(w_{t-1})}}},\\
    &= F_{m}(w_{t-1}) -\eta_t\norm{\nabla F_{m}(w_{t-1})},\\
    &\geq^{(Ass. \ref{ass:lip})} F_{m}(w_{t-1}) -\eta_tL.
\end{align*}
Assuming $\eta_t \leq \frac{\epsilon}{L}$ we get that for all $m\in[M]$,
\begin{align*}
    F_m(w_{t-1})  &\leq 3\epsilon + \epsilon,\\ 
    &= 4\epsilon,
\end{align*}
which proves the claim.
\end{proof}

==> src/conc.tex <==
In this paper, we studied the impact of agents' defections in federated learning and proposed an algorithm to avoid defections. As aforementioned in the section of Discussion, one open problem is how to extend our Algorithm \ref{alg:reweight} when only stochastic oracles are accessible. There are some other interesting future directions in the following.

\paragraph{Convergence rate.} We only provide asymptotic convergence guarantee for Algorithm \ref{alg:reweight}. The non-asymptotic guarantee is an interesting open question. The main difficulty lies in that there are several phases and we analyze each phase separately. The standard technique for analyzing first-order methods cannot be applied in this case. Furthermore, even in the asymptotic setting, we believe we can improve our precision guarantee from $4\epsilon$ to $(1+\delta)\epsilon$ for arbitrarily small $\delta$. 

\paragraph{Approximately realizable setting.} In this work, we focus on the realizable setting, where there exists $w^*\in \www$ such that $F_m(w^*) = 0$ for all $m\in [M]$. However, the next natural question to ask is: can we get similar results when $w^*$ is only approximately optimal for all agents?

\paragraph{Non-convex optimization.} We focus on the convex optimization setting. However, a natural follow-up question is how to avoid defections in non-convex federated optimization. While we perform experiments in the non-convex setting, our theory doesn't capture this setting. 

\paragraph{Other rational behaviors.} We restrict to the setting where the server cannot save the intermediate models and wants the final model to be as good as possible. It is also interesting to consider settings where the server can save multiple intermediate models and use the best one when a new agent from the population arrives.

==> src/related_work.tex <==
Designing incentive mechanisms for federated learning has recently received much attention, but it remains hard to solve. The main difficulty lies in an \textit{``information asymmetry"} \citep{kang2019incentive}. The server does not know the available computation resources and the data sizes on the devices for training. Furthermore, it doesn't know the local data quality of a device and can't estimate it using common metrics such as data Shapley \citep{ghorbani2019data} as it doesn't have access to raw data. As a result, the server may incur a high cost when providing incentives to the devices to encourage truthfulness or avoid defections. Or worse, it might not even be able to incentivize desired behavior.

In this section, we survey some recent advances in solving this problem. We divide the survey into four parts,
\begin{enumerate}
    \item In section \ref{sec:valuation}, we survey papers that tackle the problem of \textit{agent selection} based on several factors, but primarily the value of the data the agent can provide. This is an important step because for cross-device FL to work, the agents defining problem \eqref{eq:relaxed} should (i) represent the meta distribution $\ppp$ well, (ii) have enough data samples/computational power to converge to a solution for \eqref{eq:relaxed}.
    \item In section \ref{sec:collection}, we survey the papers that assume the pool of agents is fixed, but the agents are self-serving and want to contribute the least amount of data possible. This is because data collection and privacy costs are involved with sharing data. The works in this category also tackle the "free-rider" problem \citep{karimireddy2022mechanisms} so a handful of devices don't collect most of the data at equilibrium. 
    \item In section \ref{sec:csfl}, we survey papers relevant to a simpler problem called \textit{cross-silo FL} \citep{kairouz2019advances} where $\ppp$ is supported on a finite set of machines, and as a result, we can directly consider problem \eqref{eq:relaxed}. Defection is not a problem in this setting, and we are more interested in incentivizing the machines to contribute higher-quality model updates.
    \item Finally, in section \ref{sec:cdfl}, we survey the very limited work in the general problem we are interested in solving, i.e., avoiding defections in cross-device FL.
\end{enumerate}
There is another orthogonal line of research on fairness in FL (see \cite{ezzeldin2021fairfed} and the references within, for example). 

\subsection{Data valuation and agent selection}\label{sec:valuation}

There are two main series of works that are most relevant. The first one studied the design of incentive mechanisms under a principal-agent
model using contract theory. 
   
\cite{kang2019incentive} proposed a contract theory-based incentive mechanism for federated learning in mobile networks. They considered the principal-agent model that there are $M$ types of agents, where the agent's local data quality defines the type. The server does not know the type of each device and only has a prior distribution over all agent types. It aims to design an incentive-compatible mechanism that incentivizes every agent to behave truthfully while maximizing the server's expected reward.  \cite{tian2021contract} extended this model by considering the agent's willingness to participate as part of the type. As a result, they proposed a two-dimensional contract model for the incentive mechanism design. \cite{cong2020vcg} considered a similar model where the data quality and cost define the agent's type. The server decides payment and data acceptance rates based on the reported agent type. The authors proposed implementing the payment and data acceptance rate functions with neural networks and showed they satisfy proper properties such as incentive compatibility.  Another related work is by \cite{zeng2020fmore}, who proposed a multi-dimension auction mechanism with multiple winners for agent selection. The authors presented a first-price auction mechanism and analyzed the server's equilibrium state. 

Besides applying contract theory to incentivize agents' truthful behavior, there has also been another series of work that focuses on designing reputation-based agent selection schemes to select high-quality agents. Specifically, \cite{kang2019incentive} proposed a model that works as follows: the server computes the reputation of every agent and selects agents for the federated learning based on the reputation scores, and the reputation of every agent is updated by a management system after finishing an FL task, where a consortium blockchain implements the reputation management system. \cite{zhang2021incentive} extended the reputation-based agent selection scheme with a reverse auction mechanism to select agents by combining their bids and comprehensive
reputations. \cite{xu2020reputation} proposed a different reputation mechanism that computes the reputation of every agent based on the correlation between their report and the average report. Each agent will be rewarded according to their reputation, and those with low reputations will be removed. 

Finally, it is also worth mentioning two other related works. \cite{richardson2020budget} designed another data valuation method. 
They collect an independent validation data set and value data through an influence function, defined as the loss decreases over the validation data set when the data is left out. And \cite{hu2020trading} cast the problem as a Stackelberg game and choose a subset of agents, which they claim are most likely to provide high-quality data. They provide extensive experiments to test their idea. 

\subsection{Incentivizing agent participation and data-collection}\label{sec:collection}

Usually, the utility of participating agents is a function of model accuracy, computation/sample collection cost, and additional constant cost, e.g., communication cost and payment to the server. In a simple case where the model accuracy is a function of the total number of input samples, \cite{karimireddy2022mechanisms, zhang2022enabling} show that when the server gives the same global model to every agent like federated averaging \citep{mcmahan2016communication} does, a Nash Equilibrium exists for individual sample contributions. But, at this Nash Equilibrium, agents with high sampling costs will be ``free-riders" and will not contribute any data, while agents with low sampling costs will contribute most of the total data.

To alleviate this situation, \cite{karimireddy2022mechanisms} propose a mechanism to incentivize agents to contribute more by customizing the final model's accuracy for every agent, which means sending different models to different agents.
They show that their mechanism is ``data-maximizing" in the face of rational agents. \cite{sim2020collaborative} study a similar setting as \cite{karimireddy2022mechanisms} and aim to provide model-based rewards. Specifically, the authors use information gain as a metric for data valuation and show their reward scheme satisfies some desirable properties. \cite{zhang2022enabling} also study an infinitely repeated game, where the utility is the discounted cumulative utility, and propose a cooperative strategy to achieve the minimum number of free riders.

\cite{zhan2020learning} formulate the problem as a Stackelberg game, where the server decides the payment amount first, and agents decide the amount of data they are willing to contribute. The server's utility is the model accuracy minus the payment, while the agents' utility is the payment (proportional to the contributing data size) minus the computation cost. In this setting, the agents do not care about accuracy, which differs from our case.

In a bit of orthogonal work, \cite{cho2022federate} propose changing objective \eqref{eq:relaxed} itself to maximize the number of agents that benefit from collaboration. They provide some preliminary theoretical guarantees for a simple mean estimation problem. While in our setting, we assume the server can get the model from agents. \cite{liu2020incentives} study the problem of eliciting truthful reports of the learned model from the agents by designing proper scoring rules. Specifically, the authors consider two settings where the server has a ground truth verification data set or only has access to features. The authors demonstrate the connections between this question and proper scoring rule and peer predictions (i.e., information elicitation without verification) and test the performance with real-world data sets. 


\subsection{Maximizing data quality in cross-silo FL}\label{sec:csfl}

\cite{kairouz2019advances} demarcate between two prominent federated learning paradigms: cross-silo and cross-device. We have already discussed an example of cross-device Fl: training on mobile devices. Cross-silo FL captures the traditional training in data centers or between big organizations with similar interests. One example is a collaboration between medical institutions to improve their models without leaking sensitive patient information \cite{bergen2012genome}. In cross-silo FL, usually, the agents initiate the FL process and pay the central server for global aggregation. As a result, defection is not an issue in cross-silo FL because, ultimately, the goal is to develop better individual models. Unfortunately, there can still be ``free-riding" behavior in the cross-silo setting \citep{zhang2022enabling, richardson2020budget} as the devices have incentives to contribute less to maximize their own benefit. Therefore, maximizing the data quality is one of the main problems in cross-silo FL.


\cite{xu2021gradient} propose a heuristic Shapley score based on the gradient information from each agent. The score is calculated after communication by comparing the alignment of an agent's gradient with the aggregate gradient. Then the agents with a high score are provided an un-tarnished version of the aggregated gradient, while the agents with a lower score only get a noisy version of the gradient. This incentivizes devices to provide higher-quality gradient updates to get a final model close to the model of the server. There are, unfortunately, no guarantees showing this won't hurt the optimization of objective \eqref{eq:relaxed}, or it at least provably maximizes data quality in any sense. A similar idea has also been used in \cite{shi2022fedfaim}. \cite{zheng2021fl} also propose an auction mechanism modeled using a neural network that decides the appropriate perturbation rule for agents' gradients and an aggregation rule that helps recover a good final guarantee despite this perturbation. \cite{richardson2020budget} take a different approach, and instead of perturbing the model updates, they make budget-bound monetary payments to devices. Their metric is like the leave-one-out metric in data valuation but for model updates. Finally, \cite{tang2021incentive} formulate a social welfare maximization problem for cross-silo FL and propose an incentive mechanism with preliminary theoretical guarantees. 

% \subsection{Fairness in FL}
% Many recent papers have also studied fairness constraints in federated learning; for instance, see \cite{ezzeldin2021fairfed} and the references contained within.

\subsection{Towards avoiding defections in cross-device FL}\label{sec:cdfl}
There doesn't exist any theoretical work for our proposed problem, i.e., avoiding agent defection while optimizing problem \eqref{eq:relaxed} using an iterative algorithm with several communication rounds. There are, however, some empirical insights in other works.     

The most relevant work is about \textsc{MW-FED} algorithm \citep{blum2021one}, an algorithm that fits into the intermittent communication model and explicitly slows down the progress of devices closer to their target accuracies. Specifically, the algorithm asks the devices to report their target accuracies at the beginning of training. Then after each communication round, the devices report their validation accuracy on the current model. The server then uses a multiplicative weight update rule to devise a sample load for each device for that communication round. Intuitively, devices closer to their target accuracies get a lighter sample load and vice-versa. Practically this ensures that the devices are all satisfied at roughly the same point, thus avoiding any incentives to defect. While \textsc{MW-FED} hasn't been analyzed in the context of federated learning, it is well-known that it has an optimal sample complexity for optimizing distributed learning problems where the goal is to come up with a single best model for all agents, much like problem \eqref{eq:relaxed}. 
% One of our goals is to establish theoretical guarantees for \textsc{MW-FED}, perhaps in conjunction with some of the other techniques mentioned in this survey. 
% The algorithm has no in-built incentives for the agents to be truthful while reporting their accuracies.

% is point mass distribution on $((1,0),-)$, agent $2$ 's data distribution is point mass distribution on $((0,1),-)$,
% and agent $3$'s distribution put probability mass $1-2\epsilon$ on $((0,0),-)$, $\epsilon$ on $((1,1),+)$ and $\epsilon$ on $((1,1),-)$.
% If we initialize the linear predictor at all negative (i.e., linear parameter $x = (0,0)$), then agents $1$ and $2$ defect and the final output depend on whether agent $3$ samples $((1,1),+)$ more or $((1,1),-)$ more (or earlier).
% Thus, with probability $1/2$, the final model has error rate greater than $\frac{2+\epsilon}{3}$.
% While if no agents defect, we can achieve error rate $\frac{\epsilon}{3}$.
% If we initialize randomly, w.p. $1/4$, agent $1$ and $2$ will defect and there is still a chance that agent $3$ output $x=(1,1)$ and the error rate is high.



==> src/setup.tex <==
% \paragraph{Learning model} 
% \lw{somehow repeat in the introduction}
Recall that our (server's/government agency's) learning goal is to minimize $F(w) = \frac{1}{M}\sum_{m\in[M]}F_m(w)$ over all $w\in \www \subseteq \rr^d$, where $F_m(w):=\ee_{z\sim\ddd_m}[f(w;z)]$ is the loss on agent $m$'s data distribution. We assume the functions $F_m$'s are differentiable, convex, Lipschitz, and smooth. 
\begin{assumption}\label{ass:cvx_smth}
    Differentiable $F_m:\www\to\rr$ is convex and $H$-smooth, if for all $u, v\in \www$, $$F_m(v) + \inner{\nabla F_m(v)}{u-v} \leq F_m(u) \leq F_m(v) + \inner{\nabla F_m(v)}{u-v} + \frac{H}{2}\norm{u-v}^2.$$
\end{assumption}
\begin{assumption}[Lipschitzness]\label{ass:lip}
    Function $F_m:\www\to\rr$ is $L$-Lipschitz, if for all $u, v\in \www$, $$|F_m(u)-F_m(v)|\leq L\norm{u-v}.$$
\end{assumption}

Furthermore, the data distributions $\ddd_m$'s have to be ``similar'' so that all agents would benefit from collaboratively learning a single consensus model. Following~\cite {blum2017collaborative}, we capture the similarity among the agents by assuming that a single model works well for all agents.  
\begin{assumption}[Realizability]\label{ass:realizable}
    There exists $w^\star\in \www$ such that $w^*$ is the shared minima for all agents, i.e., $F_m(w^*) = \min_{w\in \www} F_m(w)$ for all $m\in [M]$. We denote the set of shared minima by $\www^\star$.
    For simplicity, we assume that $F_m(w^\star) =0$, for all $m\in [M]$.    
\end{assumption}
This assumption holds when using over-parameterized models that easily fit the combined training data on all the agents. Furthermore, when this assumption is not satisfied, it is unclear if returning a single consensus model, as usual in federated learning, is reasonable.

\begin{wrapfigure}[22]{r}{0.45\textwidth}
    \vspace{-0.5em}
    \centering
\scalebox{0.8}{\input{flowchart.tex}}
        \caption{Round $r$ of ICFO algorithms.}
    \label{fig:flowchart}
    \vspace{-3em}
\end{wrapfigure}

The learning goal is to output a model $w_R$ such that $F(w_R)\leq\epsilon$ for some fixed precision parameter $\epsilon>0$.
We denote the $\epsilon$-sub level sets of the function $F_m$ by $S_m^\star$, i.e., 
$S_m^\star = \{w\in \www| F_m(w)\leq \epsilon\}$. Then our realizability assumption implies that, $S^\star := \cap_{m\in[M]}S_m^\star \neq \emptyset$.
The learning goal can be achieved if we output $w_R\in S^*$.

% \hs{===========the following part is the old version, maybe a bit redundant=====}

% Consider the federated learning among $M$ agents, where each agent $m$ is associated with a data distribution $\cD_m$.
% For any model $w\in \www$ and any data point $z$, $f(w;z)$ is the loss of $w$ denote the loss of $w$ at point $z$.
% For simplicity, we restrict to convex losses. 
% As introduced in Section~\ref{sec:intro},
% Then for any agent $m\in [M]$, the loss $F_m(w)$ of $w$ for her is the expected loss of $w$ on her data distribution, i.e.,
% $$F_m(w):=\ee_{z\sim\ddd_m}[f(w;z)]\,.$$
% Let $\hat{F}(w) = \frac{1}{M}\sum_{m\in [M]}F_m(w)$ denote the average loss over all $M$ agents.
% Throughout the paper, we assume that there exists a model $\w^\star\in\www$ that it is simultaneously good for all the agents, i.e., $F_m(\w^\star) =0$ for all $m\in [M]$~\citep{blum2017collaborative} (called the \emph{realizable} setting).
% % our learning objective is the average loss over the set $M$ of agents, i.e.,
% % \[\hat{F}(w) = \frac{1}{M}\sum_{m\in [M]}F_m(w)\,.\]
% % For some fixed loss threshold $\epsilon > \alpha$, 
% The learning goal is to output a model $w_R$ such that $\hat{F}(w_R)\leq\epsilon$ for some fixed precision parameter $\epsilon>0$.
% We denote the $\epsilon$-sub level sets of the function $F_m$ by $S_m^\star$, i.e., 
% $S_m^\star = \{w\in \www| F_m(w)\leq \epsilon\}$.
% Then our realizability assumption implies that, $$S^\star := \cap_{m\in[M]}S_m^\star \neq \emptyset.$$

% \hs{=========end===========}

% In this work, we relax it by assuming that for some small $\alpha\geq 0$, for all $m\in[M]$, $F_m(\w^\star)\leq \alpha$. 
% \vspace{-1em}

\textbf{Intermittently Communicating First-order (ICFO) Algorithms.}
% \noindent\textbf{Intermittently communicating first-order (ICFO) algorithms.} 
We focus on intermittently communicating first-order (ICFO) algorithms such as \textsc{FedAvg}. More specifically, at each round $r\in[R]$, the server sends out the current model $w_{r-1}$ to all agents participating in the learning in this round. All participating agents $m$ query their first-order oracle \footnote{In practical implementations of these algorithms, usually the agent sends back an unbiased estimate $(\hat F_m(w_{r-1}), \nabla \hat F_m(w_{r-1}))$ of $(F_m(w_{r-1}), \nabla F_m(w_{r-1}))$. This is attained by first sampling data-points $\{z^m_{r,k}\sim \ddd_m\}_{k\in K_r^m}$ on machine $m$ and returning $\rb{\frac{1}{K_r^m} \sum_{k\in[K_r^m]}f(w_{r-1}; z_{r,k}^m), \frac{1}{K_r^m} \sum_{k\in[K_r^m]}\nabla f(w_{r-1}; z_{r,k}^m) }$. We focus on the setting with exact gradients and function values in our theoretical results but have stochasticity in our experiments.} at the current model $\ooo_m(w_{r-1}) = (F_m(w_{r-1}), \nabla F_m(w_{r-1}))$ and send it to the server, which makes an update to the model. The detailed algorithm framework is described in Figure~\ref{fig:flowchart} and Algorithm~\ref{alg:icfo} in the appendix.


Note that in the ICFO algorithm class, different algorithms can determine (i) the initialization $w_0$, (ii) step sizes $\eta_{1:R}$, and (iii) an aggregation rule $h_r(\cdot)$ for each round, which takes input $\{\ooo_m(w_{r-1})\}_{m\in \cM_r}$ and outputs a vector in $Span\{\nabla F_m(w_{r-1})\}_{m\in \cM_r}$.
For example, \textsc{FedAvg} will use uniform aggregation, i.e., set $h_r\rb{\{\ooo_m(w_{r-1})\}_{m\in \cM_r}} = \frac{1}{\abs{\cM_r}}\sum_{m\in \cM_r}\nabla F_m(w_{r-1})$ for all $r\in [R]$. We say an ICFO algorithm is \textbf{convergent} if the algorithm will converge to optima when agents are irrational, i.e., when agents never drop out.





% \hs{==================remove the following verbal description===========}

% We focus on a class of algorithms that communicates intermittently and uses iterative first-order optimization between communication rounds. 
% This class of algorithms is called intermittent-communicative first-order (ICFO) algorithms.
% This scheme includes almost all popular federated learning algorithms, e.g., \textsc{FedAvg} and \textsc{FedSGD}.

% % \begin{figure}[H]
% %     \centering
% %     \includegraphics[width=0.8\textwidth]{IC.png}
% %     \caption{Description of algorithm scheme in the ideal intermittent communication setting when no defections happen, and each agent performs the same number of local steps $K$ for $R$ communication rounds.}
% %     \label{fig:IC}
% % \end{figure}

% \begin{itemize}
%     \item \textbf{Intermittent communication.} We consider algorithms in the intermittent communication setting described by Fig~\ref{fig:IC}, which usually is composed of fours steps in each round: 1) the server sends the agents a synchronized model; 2) the agents do local updates using their local data; 3) agents send the updates to the server; 4) the server aggregates the updates and synchronizes the model.
%     We allow agents to drop out the training procedure at the beginning of each round after receiving the synchronized model.
%     When some agents drop out, the communication structure is still the same, but the number of existing agents at any round $r\in[R]$ is not $M$ anymore. 
%     Let $\cM_r$ denote the set of agents participating in communication round $r$.
%     Let $R$ denote the total number of rounds.
%     % Thus the total number of rounds $R = \min\{r\in \NN_+|\frac{1}{\abs{\cM_r}}\sum_{i\in \cM_r} F_i(w_{r-1}) <\epsilon\}$ is the earliest round when the average loss of remaining agents is smaller than $\epsilon$ and the total parallel run-time is $T=KR$.
%     Then $\cM_0=[M]$ and $|\cM_r|\geq 1$ for any $r\in R$, i.e., there is at least one agent during the optimization process. 
%     We don't allow the agents to join back once they've left. If an agent $m$ drops out during round $r$, then $m\in \cM_{r-1}\setminus \cM_{r}$.     
%     % We'd consider a slightly more general class of algorithms below where each agent can make a different number of local steps at each round $r$, say $K_r^m$.\todohs{to check if we need this notation}
    
%     % when there are no defections, there are $M$ agents that communicate for $R$ rounds and make $K$ local steps between these communication rounds.  When defections occur, the communication structure is still the same, but the number of agents at any time step $t\in[T]$ is not $M$ anymore. 
%     % Let $S_r$ denote the set of agents participating in communication round $r$. Then $S_1=[M]$ and we assume $K, R$ is such that $|S_R|\geq 1$, i.e., there is at least one machine at the end of the optimization. We also don't allow the agents to join back once they've defected. We say that an agent $m$ defected during round $r$ if $m\in S_{r-1}\setminus S_{r}$. 
%     \item \textbf{Iterative optimization as first-order local updates.} The agents use iterative optimization algorithms such as stochastic gradient descent for local model updates. In round $r$, agent $m\in \cM_{r-1}$ receives a synchronized model $w_{r-1}$ from the server and makes updates starting from $w_{r-1}$.
%     Following the instruction of the server about the step size $\eta$ and batch size $K_r^m$, agent $m$ draws $K_r^m$ i.i.d. samples \todohs{simplify the description to fit the algs considered in this work only  }$z^m_{r,1},\ldots,z^m_{r, K_r^m}\sim\ddd_m$, and then updates its local model, $$w_{r}^{m} = w_{r-1} -\eta\cdot\frac{1}{K_r^m}\sum_{k\in[K_r^m]}\nabla f(w_{r,k}^m;z_{r,k}^m),$$  where $w_{r,k}^m$ are some intermediate models at which the agent $m$ makes gradient queries for $k\in[K_r^m]$.
%     Hence, agents never communicate their raw data and exchange only gradients.
%     % Agent $i$ draw i.i.d. samples $z^{i}_1,\ldots, $ for $t\in[(r-1)K, rK-1]$ from their distributions $\ddd_m$ but never communicates these raw data.
%     % Instead, it sends a sequence of $K$ model updates $\{\nabla f(w_t^m; z^i_t^m)\}_{t\in[(r-1)K, rK-1]}$.
%     This captures various distributed optimization algorithms, such as large mini-batch SGD (\textsc{FedSGD}) \citep{dekel2012optimal} and local SGD (\textsc{FedAvg}, algorithm \ref{alg:fedavg}) \citep{mcmahan2016communication}. For instance, for large mini-batch SGD, all the local gradient queries in round $r$ are made at the point $w_{r-1}$, i.e., $w^m_{r,j} = w_{r-1}$ for all $m\in[M], j\in[K^m_{r}]$, while for \textsc{FedAvg}, the queried points may keep changing within the communication round (see Algorithm~\ref{alg:fedavg} for a version with fixed local steps). After receiving the models from the agents, the server then computes a convex combination of the models as $w_r = \text{Conv}(\{w_r^m\}_{m\in\mmm_r})$ and sends it back to all agents in $\mmm_r$.  
%      % We note that we don't allow the server to send different models to each machine after synchronization, i.e., the server can't incentivize any behavior by model differentiation. This assumption is to align with the majority of applications in cross-device federated learning, where model differentiation could affect the optimizer's convergence unpredictably. 
% \end{itemize}



% \vspace{-1.5em}
\textbf{Rational Agents.}
% \noindent\textbf{Rational agents.} 
% We consider that all
% We assume that all the $M$ agents defining the problem \ref{eq:relaxed} are \textit{``rational"}. 
Since agents have computation/communication costs to join this collaboration, they will defect when they are happy with the instantaneous model's performance on their local data.
In particular, in the $r$-th round, after receiving a synchronized model $w_{r-1}$ from the server, agent $m$ will defect permanently if the current model $w_{r-1}$ is satisfactory, i.e.,  $F_m(w_{r-1})\leq \epsilon$ for some fixed precision parameter $\epsilon>0$. Then, agent $m$ will not participate in the remaining process of this iteration, including local training, communication, and aggregation. Thus, $m\notin \cM_{r'}$ for $r'\geq r$, where $\cM_{r'}$ is the set of participating agents in round $r'$. 
Note that a sequence of agents may defect for an algorithm $\aaa$, running over a set of rational agents. We say the defection behavior (of this sequence of agents) \textbf{hurts} (for algorithm $\aaa$) if the final output $w_R\notin S^\star$, i.e., we don't find a model in the $\epsilon$ sub-level set of an otherwise realizable problem.  

In the field of game theory (and economics), the rationality of agents is commonly modeled as aiming to maximize their net utility, which is typically defined as the difference between their payoffs and associated costs, such as the difference between value and payment in auctions or revenue and cost in markets \citep{myerson1981optimal,huber2001gaining,borgers2015introduction}.
In our model, each agent aims to obtain a loss below $\epsilon$ over their local data distribution (and any loss below $\epsilon$ is indifferent), and therefore, their payoff upon receiving a model $w$ is $v(w) =V\cdot \ii[F_m(w)\leq \epsilon]$
for some $V>0$.
Their costs increase linearly with the number of rounds they participate in the training process. Therefore, the cost of participating in training for $r$ rounds is given by $c(r) = C\cdot r$ for some constant $C\ll V$.
In this case, the optimal choice for the agent is to defect once they receive a model with a local loss below $\epsilon$ and never return in the future.



% It is important to note that the agent's utility function isn't confined solely to this specific definition. We have selected this straightforward yet indicative utility function to illustrate a specific type of agent defection behavior. In this case, the agent defects when the ML model's performance surpasses a certain threshold, and once they defect, they do not return in the future.

% the utility $u_m(w, r)$ of each agent $m$ as the difference between their payoff $v\big(F_m(w)\big)$ of receiving an ML model $w$ and their cost of participating in the training, i.e., $u_m(w, r) = v\big(F_m(w)\big) - c(r)$. We assume the agent's payoff function is a threshold function, i.e., $v\big(F_m(w)\big) = \begin{cases}
%     V \quad \text{if $F_m(w) \le \epsilon$,} \\
%     0 \quad \text{otherwise.}
% \end{cases}$ The agent's cost function is defined as $c(r) = C\cdot r$, i.e., the agent suffers a constant cost $C$ at each round during the training. 
% %
% % agent $m$ defects at some point, we say the defection of agent $m$ 
% %
% % We first define ``hurtful defections'' as follows.
% % For any agent distributions $\cD_1, \cD_2, \cdots, \cD_M$ and hypothesis class $\cH$, for any $i\in [M]$, 
% % \begin{definition}
% %     Let $w^* := \argmin_{w \in \www} \hat F(w)$ denote the optimal classifier when no agents defect.
% %     Consider an algorithm $\aaa$ with final output model $w_T$ after agent $i$ defects at some point. We say the defection of agent $i$ hurts if $\hat F(w_T)>\epsilon$.
% % \end{definition}


% From a game theoretical perspective, we can view this learning problem as a repeated Stackelberg game between the server and the agents, where in each round $r$, the server (``the leader'') proposes an ML model $w$ and then the agents (``the follower'') decides whether to drop out or to stay and perform the designated task.
% If agent $m$ defects in round $r$, then her utility\footnote{Agents know their utilities when they defect but not when they stay.} is
% \begin{equation}\label{eq:agent_utility}
% u_m(w, r) = v\cdot \ii[F_m(w)\leq \epsilon] - C\cdot (r-1),
% \end{equation}
% where $v$ and $C$ represent constants that capture the model value and computation/communication costs per round.  Since the agents' primary objective is to achieve low loss on their data, $v\gg C$. The detailed process at each round is depicted in Fig~\ref{fig:flowchart} in the appendix. 

% \hs{ ==========the following is the previous version. we can remove it if you guys feel the new version is better.========}

% To capture the computation/communication cost that incentivizes agents' defections, we define the following utility function,
% \begin{equation}\label{eq:agent_utility}
% u\rb{w, \ddd, T} = v\cdot \ii[\ee_{z\sim \ddd}[f(w;z)]\leq \epsilon] - C\cdot T,
% \end{equation}
% where $T$ is the total number of samples/local updates made using distribution $\ddd$, $w$ is the model for which we evaluate the utility and $v, C$ are some constants scaling the model value and sampling/computational cost.
% In particular, if $T_r^m:= \sum_{j=1}^{r-1}K_j^m$ is the total number of local update steps (local i.i.d. samples drawn) by agent $m$, upto round $r-1$, then agent $m$'s utility at the beginning of round $r$  is $u\rb{w_{r-1}, \cD_m, T_r^m}$.
% % , and $K_r^m$ is the number of local steps performed before round $r$ by agent $m$. 
% % Note that this model differs from the intermittent communication model assumed above because the devices might be asked to do a different number of local updates. 
% Further, we assume $v>>C$, so once an accurate enough model is attained, the devices can make up for the incurred cost; however, they don't have any incentive to not deviate at that point. 

% \hs{==============end============}

% \begin{figure}
%      \centering
%           \begin{subfigure}[b]{0.69\textwidth}
         
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{defection_time.png}
%          \caption{Defection over time}
%          \label{fig:defection_time}
%      \end{subfigure}
     

%         \caption{}
%         \label{fig:defection_setup}
% \end{figure}





% \textcolor{red}{HS: put all definitions (of ``similar enough'', ``iterative alg'',``defection'', ``defection condition'') here}

==> src/why_defection_hurts.tex <==
One might naturally wonder whether defections in an optimization process are universally detrimental, consistently harmless, or fall somewhere in between for any given algorithm. Our experiments, as shown in Figure \ref{fig:defection_combined}, confirm the existence of harmful defections. However, it's worth noting that not all defections have a negative impact; some are actually benign.
\begin{observation}
    There exists a learning problem with two agents such that for any convergent ICFO algorithm $\cA$, any defection will be benign, i.e., $\cA$ will converge to a $w_R\in S^*$.
    % with $F_m(w_R)\leq \epsilon$ for all $m\in [M]$.
\end{observation}
Consider a $2$-dimensional linear classification problem where each point $x\in \R^2$ is labeled by $w^* = \ind{\be_1^\top x\leq 0}$. There are two agents where the marginal data distribution of agent $1$ is uniform over the unit ball $\{x|\norm{x}^2 \leq 1\}$ while agent $2$'s marginal data distribution is a uniform distribution over $\{\pm \be_1\}$. In this case, any linear model $w$ satisfying agent $1$, i.e., $F_1(w)\leq \epsilon$ (for any appropriate loss function) will also satisfy agent $2$. Therefore, for any convergent ICFO algorithm,  if there is a defection, it must be either agent 2's defection or the defection of both agents. In either case, the defection is benign for any convergent ICFO algorithm.
This example can be extended to a more general case where agent $1$'s $\epsilon$-sub level set is a subset of agent $2$, i.e., $S^*_1\subset S^*_2$. 


In practice, the ideal scenario where defections are benign is uncommon, as most defections tend to have a negative impact (refer to Figure~\ref{fig:defection_cartoon} for an illustration). Thus, the extent to which defections are harmful is largely algorithm-dependent. To gain insights into which algorithms can mitigate the negative effects of defections, we will explore the roles of initialization, step size, and aggregation methods in this section. These insights will inform our algorithmic design in the subsequent section. Let's consider the following example for further clarity.



% It is harder to characterize the necessary and sufficient conditions for defection to be harmful, which depends on the data distributions and algorithm. 

% One trivial condition for a \textit{``benign defection"} is that there exists an agent whose $\epsilon$-sub level set is a subset of the defecting agent's $\epsilon$-sub level set. Thus, even if the latter agent defects, the algorithm converges to the former agent's $\epsilon$-sub level set. 

% the input space $\R^2$ and all data labeled by $\ind{\be_1^\top x\geq 0}$.
% Agent $i$'s marginal data distribution is uniform over $\{\pm \be_1\}$ while agent $j$'s distribution is uniform over the unit ball. In this case, the defection of agent $i$ won't hurt because overfitting agent $j$ will not lead to a worse loss on agent $i$. 
% When 


% When one agent $i$'s task is strictly easier than another agent $j$ (which means that, for any predictor performing well under distribution $\cD_j$, it also performs well under distribution $\cD_i$), then if one of the agents $i$ and $j$ defects, it must be agent $i$. 


% \paragraph{Initialization.}

\begin{example}\label{eg:def_hurt}
    Consider an example with two agents with $\www = \R^2$,  $F_1(w) = \abs{(0,1)^\top w}$ and $F_2(w) = \abs{(1,-1)^\top w}$ as illustrated in Figure~\ref{fig:example-def}.
    Then we have the optimal model $w^* = (0,0)$ and the subgradients $\nabla F_1(w) = \sign((0,1)^\top w) 
    \cdot (0,1)$ and $\nabla F_2(w) = \sign((1,-1)^\top w)\cdot (1,-1)$. Note that the functions can be smoothed, and the following observations remain.
\end{example}
% \begin{figure}[H]
% \begin{minipage}{0.44\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{fig/eg1.jpeg}
%          \caption{Illustration of Example~\ref{eg:def_hurt}.}
%          \label{fig:example-def}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.49\textwidth}
%     \includegraphics[width=\textwidth]{fig/eg2.jpeg}
%          \caption{Illustration of the example in Observation~\ref{obs:aggre}.
%         }
%          \label{fig:aggre}
%     \end{minipage}
% \end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig/eg1.jpeg}
         \caption{Contour illustration of Example~\ref{eg:def_hurt}.}
         \label{fig:example-def}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/eg2.jpeg}
         \caption{Contour illustration of  Observation~\ref{obs:aggre}.
        }
         \label{fig:aggre}
     \end{subfigure}
        \caption{Illustrations of the contours of the examples presented in Section \ref{sec:defections_hurt}.}
        
        \label{fig:defection}
\end{figure}
% Supposing that we initialize at $w_0 =(1,1)$, then $F_2(w_0) = 0$.
% which might lead to overfitting to the remaining agents and, thus, it will be a harmful defection.
\begin{observation}
    There exists an initialization such that harmful defections are inevitable for any ICFO algorithm in Example~\ref{eg:def_hurt}. 
    Specifically, there exists a $w_0\in S_1^*\cup S_2^*$ such that for any ICFO algorithm $\cA$, when initialized at $w_0$, $\cA$ will converge to a model $w_R\notin S^*$. 
    Furthermore, there exists a $w_0\in S_1^*\cup S_2^*$ such that any ICFO algorithm initialized at $w_0$ will converge to a $w_R$ with $F(w_R) \geq 1/2 >0 =F(w^*)$.
\end{observation}
For example, if the algorithm is initialized at $w_0 = (1,1)$, agent $2$ defects given $w_0$ and an ICFO algorithm can only update in the direction of $\nabla F_1(w) = (0,\sign((0,1)^\top w))$. It will converge to a $w_R \in \{(1,\beta)|\beta\in \R\}$ and incurs $F(w_R)\geq \frac{1}{2}$ since $F(w) \geq \frac{1}{2}$ for all $w\in \{(1,\beta)|\beta\in \R\}$.
Note that if the algorithm is initialized at any point in the dotted region of Figure~\ref{fig:example-def}, which is a subset of $S_1^*\cup S_2^*\setminus S^*$, one agent would defect immediately. The algorithm can only make updates according to the remaining agent and leads to a $w_R\notin S^*$. 
We refer to the dotted region as the \emph{bad region}.
% If we initialize in one agent's $\epsilon$-sub level set, the agent will immediately defect, and then the entire optimization process will only depend on the remaining agent, and possibly lead to a harmful defection.
% Suppose that the algorithm initialize at $w = (1,1)$, then we have $F_2(w) =0$ and agent $2$ defects.
% Therefore the algorithm will optimize over $F_1$ and, thus, converge to some point in the form of $w_R = (1,1)+ (0,\alpha)$ for some $\alpha \in \R$, then either $F_1(w_R)\geq \frac{1}{2}$ (if $\alpha \geq -\frac{1}{2}$) or $F_2(w_R)\geq \frac{1}{2}$ (if $\alpha \leq -\frac{1}{2}$).
% We could show that if the initialization falls into the \tba{formula for dotted region} (the dotted region in Fig~\ref{fig:init}), then no IFCO algorithm can avoid harmful defections. 
No ICFO algorithm can avoid harmful defections when initialized in the bad region. The next question is: can specific algorithms avoid harmful defections when initialized in the good region? We then notice that we must be very careful about step sizes. 
We need to fix an aggregation method to discuss the effects of step sizes, and here we consider uniform aggregation, for example.
\begin{observation}\label{obs:stepsize}
Consider randomly choosing the initialization $w_0$ from $\{w|\norm{w}\leq 1\}$.
In Example~\ref{eg:def_hurt}, with probability $1-2\epsilon$ over $w_0$,
there exists a sequence of step sizes $\eta_{1:R}$ 
% \footnote{In Sec~\ref{sec:setup} we consider constant step-sizes, but this is w.l.o.g. since the aggregation rule can absorb any round dependent constants.} 
such that the ICFO algorithm with uniform aggregation cannot avoid harmful defections, i.e., $w_R\notin S^*$.
\end{observation}
In Figure~\ref{fig:example-def}, if we initialize at any point in the white area, we can set the step size s.t. the algorithm will converge to a $w_R\notin S^*$. For example, if we initialize at $w_1$ or $w_2$ in Figure~\ref{fig:example-def}, the algorithm will step into the bad initialization region after the update by setting step size according to the blue trajectories.
If we initialize at $w_3$ or $w_4$ in Figure~\ref{fig:example-def}, 
% if we initialize at any $w_0$ in the light gray region, 
% then we can set the step size s.t. the algorithm will step into the bad initialization region after the update (see the blue trajectory for example).
% If we initialize at any point in the dark region, e.g. $w_2$ or $w_3$ in Figure~\ref{fig:example-def}, 
then by appropriately setting the step sizes, the algorithm will follow the purple trajectory in the figure. In this case, 
the algorithm will step into $S_2^*$ after round $1$, followed by agent $2$ defecting, and eventually converge to a $w_R \in S_1^* \setminus S_2^*$.
Observation~\ref{obs:stepsize} can be extended to other aggregation methods.
If we initialize at $w_2$, except making an update in the direction towards $(2\epsilon,\epsilon)$ (which requires more than local information), there is a choice of step size s.t. the algorithm will step into the bad region.
% As illustrated in Fig~\ref{fig:example-def}, for initialization $w$ in the \tba{formula for light gray region}, 
% For $w$ in the \tba{formula for  dark gray region}, we can also design the step size to make agent $2$ defect first and converge to a point outside the $\epsilon$ sub-level set of agent $2$ as illustrated in the figure.
However, having a good initialization and carefully selected step sizes will not be sufficient.  
Any ICFO algorithm with uniform aggregation cannot avoid harmful defections.
\begin{observation}\label{obs:aggre}
    For any ICFO algorithm $\cA$ with uniform aggregation, there exists a learning problem of two agents in which $\cA$ initialized in the good region will converge to a model $w_R\notin S^*$.
    % For any ICFO algorithm $\cA$ with uniform aggregation, there exists an learning problem of $2$ agents in which, for any initialization $w_0\notin S_1^*\cup S_2^*$, $\cA$ will converge to a model $w_R\notin S^*$.
    
    % For any ICFO algorithm, there exists an learning problem in which 
    % any ICFO algorithm with uniform aggregation cannot avoid defections.

    % There exists an learning problem in which 
    % any ICFO algorithm with uniform aggregation cannot avoid defections.
    % initializing at any point in $\www\setminus (\cup_{m}S^*_m)$   with any step size and any initialization 
    % Moreover, 
    % any convergent ICFO algorithm initializing at any point in $\www\setminus (\cup_{m}S^*_m)$ with uniform aggregation with any pre-specified step size (i.e., $\eta_r$ being independent of $(F(w_{r'}))_{r'< r}$ for all $r\in [R]$) cannot avoid harmful defections.
\end{observation}
\begin{wrapfigure}{r}{0.5\textwidth}
% \begin{figure}[tbh]
    \vspace{-1em}
    \centering
    \includegraphics[width=0.5\textwidth]{fig/contour.png}
    \caption{
In this illustration, agent 1's loss function $F_1$ is piece-wise linear, while agent 2's loss function $F_2$ is quadratic. Both functions are truncated to have a minimum value of zero and smoothed. %a truncated quadratic of the form $F_2(w) = \max(a w_1^2 + b w_2^2 -1, 0)$. 
The figure highlights zero-loss regions: filled orange for $F_1$ and green for $F_2$. Their shared optimum is $w^\star$ where $F_m(w^\star) = 0$. Assumptions \ref{ass:cvx_smth}, \ref{ass:lip}, and \ref{ass:realizable} are satisfied, but Assumption \ref{ass:hetero} is not, as the gradients $\nabla F_1(w')$ and $\nabla F_2(w')$ are parallel at $w'$. Dashed contour lines indicate the $\epsilon$ level set ($F_m(w) = \epsilon$), and solid lines represent the $1$ level set ($F_m(w) = 1$). Starting from $w_0$,  any trajectory must pass the orange region to reach the $\epsilon$-sub level set of $F_2$. When the model updates to $w_t$ at time $t$, agent 1 would defect as $F_1(w_t) \leq \epsilon$. Subsequent updates follow $\nabla F_2(\cdot)$, and with a small step size, the model converges to $w_R$. This final model deviates from agent 1's $\epsilon$ level set, resulting in a poor performance with $F_1(w_R) = 1$.}
    % In this example, agent 1's loss function $F_1$ is a non-negative piece-wise linear function, and agent 2's loss function is a truncated quadratic function, in the form of $F_2(w) = \max(a w_1^2 + b w_2^2 -1, 0)$. Note that on the lower side of the piece-wise linear function $F_1$, the contour lines are more concentrated and imply a significantly steeper slope. These functions can be smoothed to satisfy the Assumptions \ref{ass:cvx_smth}. This figure shows $F_1(w) = 0$ for all $w$ in the filled orange region and $F_2(w) = 0$ for all $w$ in the filled green region.
    % Their tangent point $w^*$ is the shared minima as $F_1(w^*) = F_2(w^*) = 0$.
    % Therefore, all of Assumptions \ref{ass:cvx_smth}, \ref{ass:lip}, \ref{ass:realizable} hold. Assumption \ref{ass:hetero} does not hold here as $\nabla F_1(w')$ is parallel to $\nabla F_2(w')$ at $w'$.  The dashed contour lines represents the $\epsilon$ level set (i.e., $F_m(w) = \epsilon$) and the solid contour lines represents $1$ level set (i.e., $F_m(w) = 1$). Let's consider initializing at $w_0$. Any trajectory must pass the filled orange region to reach the $\epsilon$-sub level set of $F_2$. At time $t$, the model is updated to $w_t$ and agent 1 defects since $F_1(w_t) \leq \epsilon$. Then the algorithm will only update in the direction of $\nabla F_2(\cdot)$. When the step size is small, the trajectory after time $t$ is illustrated as the blue dots, and the model will converge to $w_R$. The final model $w_R$ deviates from agent 1's $\epsilon$-sub level set and performs poorly on the defected agent (in the example, $F_1(w_R) = 1.0$).
    %}
    \label{fig:defection_example}
    \vspace{-1em}
% \end{figure}    
\end{wrapfigure}
We construct a slightly different example from Example~\ref{eg:def_hurt}.
As illustrated in Figure~\ref{fig:aggre}, we consider a set of problems $\{F_1(w) = \max((0,1)^\top w,0), F_2(w) = \max((1,-1)^\top w+\alpha,0)|\alpha \geq 0\}$. For all $\alpha \geq 0$ illustrated in Figure~\ref{fig:aggre}, the problem characterized by $\alpha$ is denoted by $P_\alpha$.
Suppose we initialize at a $w_0$ which is not in the union of $\epsilon$-sub level sets $S_1^*\cup S_2^*$ of $P_\alpha$ for all $\alpha$. Otherwise, the initialization will lie in the bad region of $P_\alpha$ for some $\alpha$.
W.l.o.g., suppose the algorithm initializes at $w_0= (2,1)$.
When no agents defect, the average gradient $\nabla F(w) = (1/2,0)$ is a constant, and any ICFO algorithm can only move in the direction of $(-1,0)$ until agent $2$ defects.
Among all choices of $\alpha$, agent $2$ will defect earliest in the problem $P_0$ (since any model good for agent $2$ for some $\alpha>0$ is also good for agent $2$ for $\alpha = 0$).
The algorithm will follow the purple trajectory in Figure~\ref{fig:aggre}. 
Before agent $2$'s defection, the algorithm's updates are identical for all $\alpha \geq 0$. 
Denote by $r_0$ the round at which agent $2$ is defecting in $P_0$.
Then there exists an $\alpha'$ (illustrated in the figure) s.t. $w_{r_0}$ lies in the bad region of problem $P_{\alpha'}$.
Therefore, in problem $P_{\alpha'}$, the algorithm will output a $w_R\notin S^*$. Especially, we have $F(w_R) = 1/2 >0=F(w^*)$.

% , then $w_{r_0-1} = (c,1)$ for some $c>1+\epsilon$.
% At the end of round $r_0$, the model is updated to $w_{r_0} =(c-\eta_{r_0}, 1)$.
% Agent $2$ defects in $P_0$ and thus $c-\eta_{r_0}\leq 1+\epsilon$.
% There exists an $\alpha'$ s.t. $2\epsilon-\alpha' < c-\eta_{r}/2 \leq 1+\epsilon -\alpha'$ and in this case, $w_{r_0}$ is in the bad region of problem $P_{\alpha'}$.
% Therefore, in problem $P_\alpha$, the algorithm will output a $w_R\notin S^*$.

Note that we can avoid defections by non-uniform aggregation. For example, when the algorithm reaches a $w$ with low $F_2(w)$ and high $F_1(w)$, we can project $\nabla F_1(w)$ into the orthogonal space of $\nabla F_2(w)$ and update in the projected direction. Figure~\ref{fig:aggre} provides a visual representation of the effectiveness of the projection technique, which is shown by the black trajectory within the context of this example. This not only showcases the benefits of projection but also serves as a motivation behind the development of our algorithm.  
%As illustrated in Figure~\ref{fig:aggre}, the black trajectory illustrates the effectiveness of projection in this example. This also motivates our algorithm design.
% for At the round right before agent $2$ defects in the case of $\alpha = 0$, $w_r = (c,1)$ for some $c>1+\alpha$.

% Suppose that at round
 

% for any step size 

% Since $\nabla F_1(w)$ is either $(0,1)$ or $(0,-1)$ for all $w$, $w_R$ should be in the form of $(1,1-\alpha)$ and thus, it is close to $(1,0)$.




% \hs{=========================below is the old version ===============}

% Then we are wondering: \textbf{What optimization algorithms can avoid harmful defections altogether?}
% To understand this question, we start by analyzing the effects of different components of the algorithms and showing that what algorithms cannot avoid harmful defections.
% \paragraph{Hyper-parameters matter.}
% % The next question is: \textbf{do specific optimization algorithms avoid defections altogether?}
% % Can we disincentivize defections via tuning hyper-parameters, e.g., step and batch sizes? 
% Consider the one-dimensional two-agent example in Figure \ref{fig:learning_rate}. Assume the optimizer is initialized at $0$, with a \textit{``smal''} step size. As the iterates move towards the right, they first enter the set $S_1^\star$, then agent one defects, and the iterates proceed into $S^\star$. At this point, the optimization stops because agent two is happy with the model. Thus the final model is in $S^\star$, and defection doesn't hurt. However, for the same example, if the step size is \textit{``large"} enough so that the iterates first enter the set $S_1^\star$, agent one defects, and then they directly enter $S_2^\star\setminus S^\star$ by passing $S^\star$. In this case, the final model is not in $S^\star$, which means the defection hurts. This example illustrates that whether they hurt depends on the hyper-parameter choice of an optimization algorithm.

% \begin{figure}[tbh]
%     \centering
%     \includegraphics[width=0.7\textwidth]{learning_rate.jpg}
%     \caption{We consider two devices with $\epsilon$ sublevel sets $S^*_1$ (blue) and $S^*_2$ (red) as shown in the one dimension. $S^*$ is the sub-level set for satisfying both clients.}
%     \label{fig:learning_rate}
% \end{figure}
% % \todohs{is it necessary to define this by ``$\exists j$,...'' or $F_i(w_T)> F_i(w^*)$ is enough? I do think $t\rightarrow \infty$ is necessary since finite $T$ does not guarantee converging to opt solution. }
% %
% % Let us first describe the optimization setting. Recall that we want to optimize \eqref{eq:relaxed}, an objective defined over $M$ machines. We want to solve this problem in the intermittent communication setting \citep{woodworth2018graph}, i.e., optimization happens over $R$ communication rounds, and agents can make several local updates between the communication rounds, which are aggregated in some manner before the next round. The most common local update procedure involves running some steps of stochastic gradient descent (SGD) on each machine. When each machine makes the same number of steps, the algorithm is known as \textsc{FedAvg} or local SGD \citep{mcmahan2016communication}. 
% %

% % In particular, in the intermittent communication model, the agents decide if they want to defect after each communication round once they receive the aggregate model from the last round. 
% % We formalize the effect of the defections next. 
% % We first provide a simple example with two agents where defection happens and incurs a high expected (over machines) error rate.

% %
% \paragraph{Aggregation method matters}
% Then we wonder, can we avoid harmful defections if we choose the correct hyper-parameters including small stepsize, for specific algorithms, e.g., \textsc{FedAvg} or \textsc{FedSGD}?
% We provide another example in Fig~\ref{fig:aggregation} showing that even with small step size, defections might still hurt for any aggregation of averaging gradients of all agents. 
% Consider another example where $F_1(w) = 100\max(1-w_1, 0)$ and $F_2(w) = \max(w_1-w_2+\alpha, 0)$ for some $\alpha>0$ for $w\in \www =\{\R^2\}$. Suppose we are initialize at $\bZero$.
% At each round before any defection, we will move in the direction of $(99, 1)$ which is scaling to the average of the gradients of two agents.
% In this example, by running an algorithm using average aggregation and small stepsize, we will first reach some $w$ close to $(1,\frac{1}{99})$, then agent $1$ defects and we converge to some $w_R\approx (\frac{50}{99}-\frac{\alpha}{2},\frac{50}{99}+\frac{\alpha}{2})$, which does not satisfy agent $1$.
% \begin{figure}[tbh]
%     \centering
%     \includegraphics[width=0.5\textwidth]{fig/aggregation}
%     \caption{tba}
%     \label{fig:aggregation}
% \end{figure}
% The only step size that can avoid defection need to be very large and scale with $\alpha$ such that at the first time we step into the $\epsilon$-sub level set,  we must reach some point $w = (s,\frac{s}{99})$ s.t. $s\geq \frac{2+\alpha}{100}$ (farther than point $a$ in the figure). Since $\alpha$ can be arbitrarily large, there does not exists a step size working for all $\alpha$.
% But in this example, aggregating over normalized gradients will work. \lw{not clear}


% % we might wonder if a harmful defection can always be avoided by choosing the correct step size (in the above example, a small enough step size) for an iterative optimization algorithm.
% % -introduce unnormalized vanilla aggregation does not work
% \paragraph{Initialization matters}
% There are some $w$ that is good for some agent $i$ but bad for others.
% If we initialize at such $w$, then agent $i$ would defect in the first round.
% As shown in the previous example, if we initialize at some $w$ on the segment between point $c$ and $a$, the defection of agent $1$ would hurt any intermittent communication algorithm.

% More formally,  we provide a binary classification example where harmful defection happens in any intermittently communicating first-order algorithm with any hyper-parameter choices, and the final model is arbitrarily bad. Recall that it's common to run optimization over a surrogate loss for binary classification tasks.
% % Most surrogate losses for binary class, e.g., hinge loss, log loss, etc., can be written in the form of $f(w;(x,y)) = \ell_y(w^\top x)$, where $\ell_y(\cdot)$ is convex and $\ell_y'(v) >0$ when $\abs{v}>0$.

% % \todohs{Roughly below is the new proposition. Could you guys double check if the new proposition makes sense and the proof?
% % I am also thinking about making it more general, in the sense of making it work for a general class of surrogate loss if needed.}
% \begin{proposition}\label{prop:hardness}
% For any $M\in \NN$, there exists an example of linear classification over $M$ agents in the realizable setting (i.e., there exists $w^*$ s.t. $F_m(\w^\star) =0$ for all $m\in [M]$) satisfying that
% % satisfying that 1) realizability; 2) 
% % harmful defection: if there exists a set $A$ of agents defecting, there exists a $w$ minimizing the average loss over the remaining agents,  $w = \argmin_{w'\in \www} \sum_{m\in [M]\setminus A} F_m(w')$ such that $\hat F(w)\geq \frac{1}{2M}$.
% for any agent $m$, there exists an initialization such that the final output $w_R$ of any intermittent communication algorithm has $F_m(w_R)>3.6$.
% \end{proposition}

% \begin{proof}
% Consider $M=3$ first.
% Let hypothesis class be $3$ dimensional halfspaces $\cH = \{\ind{w^\top x \geq 0 }|w\in \R^3\}$.
% % In the following discussion, we will use $w$ to represent the hypothesis $\ind{w^\top x \geq 0 }$. 
% Consider hinge loss $f(w;(x,y)) = [1-y(w^\top x)]_+$.
% For any $m\in [3]$, agent $m$'s data distribution $\cD_m$ is the point mass distribution on $(u_m,1)$, where $u_m$ is the vector with the $m$-th entry being $1$, the $(m \mod 3 +1)$-th entry being $-0.9$ and the remaining entry being $0$.
% Then there exists a classifier $w^* = 10\cdot \bOne$ such that $F_m(w^*) = 0$ for all $m\in [3]$.
% Since all three agents are symmetric, we only need to prove the proposition for agent $1$.
% We initialize at point $w_0 = (1,0,10)$, then agent $1$ and $3$ defects in round $1$. Hence the algorithm will only run over agent $2$. The final output will be in the form of $w_R = (1, t, 10-0.9t)$ for some $t$ such that $w_R^\top u_2 \geq 1-\epsilon$.
% For any $\epsilon \leq 1$, $t$ must be greater than $4$.
% Then $w^\top u_1 < -2.6$. Hence $F_1(w_R)> 3.6$.
% The construction can be directly extended to general $M$ by letting agent $m$'s data distribution $\cD_m$ be the point mass distribution on $(u_m,1)$, where $u_m\in \R^M$ has the $m$-th entry being $1$, the $(m \mod M +1)$-th entry being $-0.9$ and other entries being zeros.
% To prove the proposition for agent $1$, we initialize at $w_0 = (1,0,10,\ldots,10)$ and then all agents will defect in round $1$. Then we can have the same result as $M=3$.
%
% Let hypothesis class be $M$ dimensional halfspaces $\cH = \{\ind{w^\top x \geq 0 }|w\in \R^M\}$.
% In the following discussion, we will use $w$ to represent the hypothesis $\ind{w^\top x \geq 0 }$. 
% For any $i\in [3]$, agent $i$'s data distribution $\cD_i$ puts probability mass $\frac{1}{2}$ on $(\bZero, 1)$, $\frac{1}{2}$ on $(\be_i+ \epsilon \be_{i \mod M+1},1)$, where $\be_i$ is the standard base vector of $\R^M$.
% Then there exists a classifier $w^* = \bOne$ such that $F_i(w^*) = 0$ for all $i\in [M]$.
% Then if there exists some agent defecting, there must exists an agent $i$ such that $i$ is not defecting but $i\mod M+1$ is defecting and an agent $j$ such that $j$ is defecting but $j\mod M+1$ is not. Therefore, the classifier $w$ minimizing the average loss over the remaining agents would have $w_{i\mod M +1} = -1$ and $w_{j\mod M +1} = 1$. Thus $F_{i\mod M +1} \geq \frac{1}{2} - \alpha$ and $F_{j} \geq \alpha$. Hence the average loss $\hat F(w)\geq \frac{1}{2M}$.
% If there are agents defecting, there are two cases. First, there is only one agent defecting. W.l.o.g., assume that agent $1$ defects. Then the classifier $w$ minimizing $F_2(w)+F_3(w)$, i.e., $w=(-1,1,1)$, has $F_1(w) = \frac{1}{2}$.
% Thus, the average loss $\hat F(w) \geq \frac{1}{6}$.
% Second, there are two agents defecting, saying agent $1$ and $2$ w.l.o.g.
% Similarly, any classifier $w$ minimizing $\err_{\cD_3}(w)$ will have $w_1\leq -1$ and $w_3 \geq  1$ and thus the average loss $\hat F(w) \geq \frac{1}{6}$.
% We complete the first part of Proposition~\ref{prop:hardness}.
% Now we consider running \textsc{FedAvg}.
% The gradient of $\ell$ is $-(2y-1)x$ when $(2y-1)w^\top x<1$.
% For any agent, w.l.o.g., agent $1$, with constant probability, agent $1$ samples $(\be_1,1)$ and the other two agents sample $(\bOne,1)$ in the first round. 
% After this round, the synchronized model $w_t = (\frac{4}{3},\frac{1}{3},\frac{1}{3})$.
% Then $F_1(w_t) = \frac{4\alpha}{3}$ and agent $1$ defects.
%\end{proof}
%
%
% \idea{We want to extend the above proposition to a general theorem.}
%
% Proposition \ref{prop:hardness} shows an instance of harmful defection, where the agents' defection causes a $\Omega(1)$ lower bound on the loss; this is in stark contrast to the $\epsilon$ learning result when defection does not happen. This result stems from the hardness of overfitting when one agent defects. 
% And this harmful defection result holds for any intermittent communicating algorithm with any choice of hyper-parameters.
% We should also notice that, Proposition~\ref{prop:hardness} depends on a specific initialization. Then we are curious about \textbf{how big the chance of a bad initialization is}. 
% \todohs{use this example to discuss more on the initialization. 
% We can have a proposition like, for any prior distribution over initialized parameters, for any small $\delta >0$, there exists an example such that w.p. $1-\delta$ over initialization, for any algorithm with any hyperparameter, a harmful defection will occur. 
% } 
% \begin{proposition}
%     For any $\gamma > \epsilon$, there exists an example with bounded $\www$ in which if the initialization $w_0$ is drawn from the uniform distribution over $\www$, then with constant probability (over $w_0$), the output of any intermittently communicating algorithm satisfies that $F_1(w_R)\geq  \gamma$.
% \end{proposition}
% \begin{proof}
%     The example is illustrated in Figure~\ref{fig:iterative_defection}.
% \end{proof}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\textwidth]{eg_init.jpg}
%     \caption{We consider two agents with $\epsilon$ sub-level sets $S^*_1$ and $S^*_2$ as shown in the 2D space. 
%     $S^*_2$ is the slab between the dashed lines and $S^*_1$ is the dashed circle and inside.
%     $F_1(w) = 0$ for all $w$ inside the solid circle.
%     $F_2(w) = 0$ for all $w$ on the solid line.
%     Hence, $w^*$ is a perfect model for both agents.
%     For all $w_0$ lying in grey region, agent $1$ will defect in round $1$ and any algorithm trained only on agent $2$ will leads to $F_1(w_R) \geq \gamma$.
%     % Note that the $S^*$ is the tangent point of these two solution spaces.  As a result, except for the zero-measure set highlighted by the dashed red line, one agent's defection (e.g., agent 1 defects at the blue point) will result in a convergence point that is not in $S^*$ and can be arbitrarily bad for $\mathcal{D}_1$.
%     }
%     \label{fig:iterative_defection}
% \end{figure}

% % \begin{proposition}
% %     Let $w^* = \argmin_{w \in \www} \hat F(w)$ denote the optimal classifier when no agents defect.
% % For any algorithm, $\aaa$, assume a subset of clients $\kkk\subset [M]$ defect. Then if this defection hurts, then for each $i\in[\kkk]$ there exists a subset of agents $S\subseteq [M]\setminus \{i\}$ such that for any $w' \in \argmin_{w\in \cH}\frac{1}{\abs{S}}\sum_{j\in S}f_{\cD_j}(w)$, $f_{\cD_i}(w')> f_{\cD_i}(w^*) $.
% % \end{proposition}
% % \begin{proof}
% %     The proof follows from the contrapositive statement and the definition of a harmful defection. 
% % \end{proof}
% In Figure \ref{fig:iterative_defection},
% once we get trapped in the grey region, agent $1$ will defect and any algorithm will converge to a $w_R$ with high $F_1(w_R)$.
% This is no way to get rid of this issue if we initialize at a model in this region.
% So, we need to make further assumptions, such that we will not fall into this region at the beginning.
% Then we propose a different aggregation way to disincentive defection.
% We also discuss how other algorithmic techniques can be used to artificially slow down agents converging quickly to their solutions along with a payment scheme that avoids defections altogether.    


 
% % In, we provide an example where any iterative optimization procedure will have defections no matter the learning rate used. This illustrates that simple fixes through hyper-parameter tuning might now work. In the next section, we discuss how other algorithmic techniques can be used to artificially slow down agents converging quickly to their solutions along with a payment scheme that avoids defections altogether.    



% % Admittedly we have not fully characterized the interplay between data, defections, algorithms, and hyper-parameters. We hope to formalize these intuitions further in the future. 

% % any agent $i$'s support of the distribution is a subset of some other agent $j$' support, if one of agents $i$ and $j$ would defect, then it must be agent $i$ b

% % the defection of the agent with a subset support would cause an 
% % overfitting problem.


% % However, it is obvious that when any agent's support of the distribution is a subset of some other agents' supports, the defection of the agent with a subset support would cause an 
% % overfitting problem.\todohs{would not cause an overfitting problem in this case?} 


% % \idea{We want to fully characterize the conditions (relationships between data distributions) under which defection hurts.}
% % Recall our definition of iterative algorithms. 
% % \begin{definition}
% % % An iterative algorithm $\cA$, at each time step $t$, queries a small batch of i.i.d. samples from the collaborating agents and then updates the current model $w_{t-1}$ to a new model $w_t$.
% % % The algorithm can decide how to assign sample burden to different agents but can only store the updated model.
% % An iterative algorithm is optimal if for any set of distribution $\cD_1, \cD_2, \cdots, \cD_M$, $w_t\rightarrow \argmin_{w \in \cH} \sum_{j\in [M]}f_{\cD_j}(w)$ as $t\rightarrow \infty$.
% % \end{definition}

% % \begin{conjecture}
% % %For agent distributions, $\cD_1, \cD_2, \cdots, \cD_M$,
% % %and a target function $f^* \in \mathcal{F}$, the defection always happens in the worst case if there exists some distributions $D_i$ and $D_j$ whose margin maximizing objective function $f_i$ and $f_j$ are different. 
% % %\textcolor{red}{
% % For any agent distributions $\cD_1, \cD_2, \cdots, \cD_M$ and hypothesis class $\cH$, let $w^* = \argmin_{w \in \cH} \\ \sum_{j\in [M]}f_{\cD_j}(w)$ denote the optimal classifier when no agents defect.
% % For any agent $i$, the defection of agent $i$ would be harmful iff there exists a subset of agents $S\subseteq [M]\setminus \{i\}$ such that for any $w' \in \argmin_{w\in \cH}\frac{1}{\abs{S}}\sum_{j\in S}f_{\cD_j}(w)$, $f_{\cD_i}(w')> f_{\cD_i}(w^*) $.
% % \end{conjecture}
% % \begin{proof}
% %     If defection hurts an agent, such a set must exist: we can show this easily by showing the contrapositive.
% %     If such a set $S$, we can construct an optimal iterative algorithm.
% %     Let $w^*_i \in \argmin_{w\in\cH} f_{\cD_i}(w)$.
% %     Then we can design an algorithm initialized at $w_0 = w^*_i$ and with the first $M-\abs{S} - 1$ updates being $w^*_j$ for each $j\in [M]\setminus(\{i\}\cup S)$ and $w_t = w'$ for the following iterations.\todokkp{is this iterative algorithm a bit stylized? It might not even be zero-respecting...}\todohs{I am ok with removing it}
    
% %     % If such a set exists, will defection necessarily hurt? No, it depends on the set and how many agents need to defect to get down to it. This makes it clear that the order in which agents leave and the point in training is also relevant.
% %     % \todokkp{Somehow, the view of just running ERM is not correct because one would be done in a single round in this view, and there is no issue of defection, we need to understand this better.} 
% % \end{proof}

% % \idea{We'd like to make progress towards proving this conjecture or refining it further.}

% % \noindent After characterizing the harmful defections, in the next section, we aim to provide a solution to disincentive such defections.
% %the next question is: how to design algorithms to disincentive such defections.


% %\todomh{....With the above lemma in mind, we should discuss when defections do and do not happen. Also, how to value each distribution and check whether these properties are satisfied? @Minbiao, do you wanna take a pass at this?....}

